Metabolic fluxes and value production

Metabolic fluxes in cells are governed by physical, physiological, and economic principles. Here I assume an optimal allocation of enzyme resources and postulate a general principle for metabolism: each enzyme must convert less valuable into more valuable metabolites to justify its own cost. The "values", called economic potentials, describe the individual contributions of metabolites to cell fitness. Local value production implies that the cost of an enzyme must be balanced by a benefit, given by the economic potential difference the catalysed reaction multiplied by the flux. Flux profiles that satisfy this principle - i.e. for which consistent potentials can be found - are called economical. Economical fluxes must lead from lower to higher economic potentials, so certain flux cycles are incompatible with any choice of economic potentials and can be excluded. To obtain economical flux profiles, non-beneficial local patterns, called futile motifs, can be systematically removed from a given flux distribution. The principle of local value production resembles thermodynamic principles and complements them in models. Here I describe a modelling framework called Value Balance Analysis (VBA) that uses the two principles and yields the same solution as enzyme cost minimisation (in kinetic models) and flux cost minimisation (in FBA). Given an economical flux distribution, kinetic models in enzyme-optimal states and with these fluxes can be constructed systematically. VBA justifies the principle of minimal fluxes and the exclusion of futile cycles, predicts enzymes that could be plausible targets for regulation, provides criteria for the usage of enzymes and pathways, and explains the choice between high-yield and low-yield flux modes.

==> files/mySIsettings.tex <==
\renewcommand{\thesection} {S\arabic{section}}
\renewcommand{\thefigure}  {S\arabic{figure}}
\renewcommand{\thetable}   {S\arabic{table}}
\renewcommand{\theequation}{S\arabic{equation}}


==> files/mysettings_arxiv.tex <==
% ------------------------------------------
% this is like in ``mysettings.tex''

\usepackage{setspace} 
\onehalfspacing
\renewcommand{\familydefault}{\sfdefault}

\usepackage{wrapfig}
\usepackage{enumitem}
\usepackage{xr}
\usepackage{color}
\usepackage{amsmath,amsfonts,amssymb}
\usepackage{epsfig}
\usepackage{graphicx}
\usepackage{colortbl}
\usepackage{url}

\definecolor{grey}{rgb}{0.9, 0.9, 0.9}

\newcommand{\remember}[1]{\marginpar{\tiny #1}}
\newcommand{\myparagraph}[1]{\vspace{-3mm}\paragraph{#1}}

\newenvironment{myitemize}{\vspace{-4pt}\begin{itemize}[leftmargin=5mm]\itemsep -2pt}{\end{itemize}}

\newtheorem{mydefinition}{Definition}
\newtheorem{mytheorem}{Theorem}
\newtheorem{mycorollary}{Corollary}

\setlength{\parindent}     {0cm}
\setlength{\parskip}       {0.2cm}
\setlength{\textwidth}     {16.5cm}
\setlength{\textheight}    {25cm}

\newcommand{\mybox}[1]{\fbox{\parbox{16.5cm}{\begin{center}\parbox{15.5cm}{#1}\end{center}}}}

% ------------------------------------------
% this is different from mysettings.tex

\newcommand{\coout}[1]{}
\newcommand{\co}   [1]{}
\newcommand{\todo} [1]{}
\newcommand{\wolf} [1]{}

\setlength{\headsep}       {-2cm}
\setlength{\oddsidemargin} {-0.3cm}
\setlength{\evensidemargin}{-0.3cm}

% \setlength{\textwidth}     {15.5cm}
% \setlength{\textheight}    {22cm}
% \setlength{\oddsidemargin} {0.3cm}
% \setlength{\evensidemargin}{0.3cm}

\pdfoutput=1
\usepackage{hyperref}
\hypersetup{colorlinks = true, allcolors = {blue}}



==> files/mysettings_arxiv_nohyperref.tex <==
% ------------------------------------------
% this is like in ``mysettings.tex''

\usepackage{setspace} 
\onehalfspacing
\renewcommand{\familydefault}{\sfdefault}

\usepackage{wrapfig}
\usepackage{enumitem}
\usepackage{xr}
\usepackage{color}
\usepackage{amsmath,amsfonts,amssymb}
\usepackage{epsfig}
\usepackage{graphicx}
\usepackage{colortbl}
\usepackage{url}

\definecolor{grey}{rgb}{0.9, 0.9, 0.9}

\newcommand{\remember}[1]{\marginpar{\tiny #1}}
\newcommand{\myparagraph}[1]{\vspace{-3mm}\paragraph{#1}}

\newenvironment{myitemize}{\vspace{-4pt}\begin{itemize}[leftmargin=5mm]\itemsep -2pt}{\end{itemize}}

\newtheorem{mydefinition}{Definition}
\newtheorem{mytheorem}{Theorem}
\newtheorem{mycorollary}{Corollary}

\setlength{\parindent}     {0cm}
\setlength{\parskip}       {0.2cm}
\setlength{\textwidth}     {16.5cm}
\setlength{\textheight}    {25cm}

\newcommand{\mybox}[1]{\fbox{\parbox{16.5cm}{\begin{center}\parbox{15.5cm}{#1}\end{center}}}}

% ------------------------------------------
% this is different from mysettings.tex

\newcommand{\coout}[1]{}
\newcommand{\co}   [1]{}
\newcommand{\todo} [1]{}
\newcommand{\wolf} [1]{}

\setlength{\headsep}       {-2cm}
\setlength{\oddsidemargin} {-0.3cm}
\setlength{\evensidemargin}{-0.3cm}

% \setlength{\textwidth}     {15.5cm}
% \setlength{\textheight}    {22cm}
% \setlength{\oddsidemargin} {0.3cm}
% \setlength{\evensidemargin}{0.3cm}


==> files/symbols_trivial_names.tex <==
\renewcommand{\cintv}{\cv}
\renewcommand{\cextv}{\sv}
\renewcommand{\Next}{\Smat}
\renewcommand{\Nint}{\Nmat}
\renewcommand{\NR}{\Nmat_{\rm R}}


==> sec_flux_analysis_FCM.tex <==
\iftoggle{bookversion}
{\section{Flux cost minimisation and economic  constraints}}
{\subsection{Flux cost minimisation and economic  constraints}}

\myparagraph{\ \\Flux cost minimisation} Classical FBA may yield flux
solutions that contain cyclic or futile cycles. In flux cost
minimisation such solutions are excluded by penalising large {\flow}s. To
do so, FCM considers all feasible {\flow}s that realise a given flux
benefit, and selects the {\flow} (or the possible {\flow}s) with a minimal
flux cost. The biological intuition is that large fluxes require large
enzyme levels, which should be avoided unless they are required by the
metabolic objective.  FBA with minimal fluxes uses a simple flux cost
function, the sum of absolute fluxes. The FBA constraints
(\ref{eq:fbastationarity}) define a polytope \coout{$\fbaPolytope$} of
feasible {\flow}s; \co{is this the F-polytope? what about flux patterns?
  rethink the terminology!} by fixing a flux benefit
($\bvtotweight\cdot \vv=b'$), we obtain a lower-dimensional the
B-polytope. \co{wort gut? was ist mit fixed flux pattern?}  From this
polytope, we can pick the {\flow}s that minimise the sum of fluxes
$|\vv|_{1}$. Alternatively, we can minimise a weighted sum of fluxes
or more general flux cost functions \cite{lieb:14a} satisfying
$(\partial \acostvl/\partial v_l)\,v_l >0$ whenever $v_l \ne 0$.  More
realistic flux cost functions (called ``enzymatic flux cost'') can be
derived from kinetic models \cite{lieb:18fcm}: we require that our
fluxes must be realised by a suitable (cost-minimising) choice of
enzyme and metabolite concentrations.  Each choice has a certain cost, which
typically increases with the enzyme and metabolite concentrations. The minimal
achievable cost defines the enzymatic flux cost of this {\flow} (or the
kinetic cost, if metabolite costs are also considered).

\myparagraph{{Economic \fluxbenefitbalance} derived from in flux cost
  minimisation} \co{adjust this with cba lagrange} \co{are kuhn-tucker
  conditions discussed here?}  In flux cost minimisation, the aim is
to find a flux distribution $\vv$ with a predefined benefit
$\bvtotweight\cdot \vv$ and a minimal flux cost $\fluxcost(\vv)$.
\coout{ (see Figure \co{\ref{fig:lagrange3}} (c)).} The fluxes, our
free variables, are constrained to a flux polytope defined by
stationarity condition and flux signs (for example, without loss of
generality we can assume that fluxes are positive).  \coout{ (dh
  welche oek var sind zu erwarten)?  wo taucht das problem auf?}  For
the  cost function $\acost(\vv)$, we require that  fluxes $v_l$ and  derivatives
$\acostvl = \partial \acost/\partial v_l$   have
the same signs (i.e.~$\acostvl\,v_l>0$), except for vanishing
fluxes $v_l=0$
where the cost function has a kink.
Linear cost function, like the sum of absolute fluxes
$\fluxcost(\vv) = \sum_l |v_l|$, are common in FBA; more
realistic, nonlinear flux costs can be derived from kinetic
models
\cite{nfbd:16}. \coout{ (see Figure \co{\ref{fig:lagrange3}} (c)).}
\coout{mention special case thermodyn (below)} \coout{All these
  optimality problems lead to economic balance equations.}
Given a flux cost function, we can consider several optimisation
scenarios. First, we may minimise the flux cost under constraints
(stationarity condition $\Nint\,\vv=0$ and fixed benefit
$\bvtotweight\cdot\vv=b$).  Using Lagrange multipliers $\omega_i$ and
$\beta$, the necessary optimality condition (for a maximal
negative flux cost) read
\begin{eqnarray}
 0= - \frac{\partial \acost}{\partial v_l} + \sum_i\, \omega_i\,  n_{il} + \beta\,\bvtotweightl,
\end{eqnarray}
and thus 
\begin{eqnarray}
[\underbrace{\beta\, \bvtotweightl}_{\bvtotl} + \sum_i \underbrace{\omega_i}_{\winti}\, n_{il} ]\,v_l
= \underbrace{\frac{\partial \acost}{\partial v_l} v_l}_{\hudotl>0}.
\end{eqnarray}
This is the reaction balance
$ \left[\Deltar \wintl + \bvtotl \right]\,v_l = \hudotl$, with the
{\enzymecost}
$\hudotl= \frac{\partial \acost}{\partial v_l} v_l = \frac{\partial
  \acost}{\partial \ln v_l}$. In a second scenario, we predefine the
production or consumption rates of some external metabolites, while
other external rates (e.g.~biomass production or nutrient uptake) can
be treated as a second objective (from which the added flux cost
function will be subtracted). We obtain the optimality condition
\begin{eqnarray}
 0= \frac{-\partial \acost}{\partial v_l} 
+ \sum_{i \in \mbox{int}} \omega^{\rm int}_i\ n_{il} 
+ \sum_{j \in \mbox{fixed}} \omega^{\rm ext}_j\, n_{jl} - \sum_{j \in \mbox{opt}} b_j\, n_{jl},
\end{eqnarray}
with Lagrange multipliers $\omega^{\rm int}_i$ (for internal
metabolites) and $\omega^{\rm ext}_j$ (for external metabolites with
fixed production rates) and benefit weights $b_j$ (for external
metabolites whose production rates are scored by the fitness
function).  After collecting $\omega^{\rm int}_i$,
$\omega^{\rm ext}_j$, and $b_j$ in one vector $\winti$, we obtain the
reaction balance equation
\begin{eqnarray}
\label{eq:irgendneGleichungA}
\sum_i \wtoti\, n_{il} \,v_l = \Deltar \wtotl\,v_l = \hudotl.
\end{eqnarray}
Note that the {\enzymecost} $\hudotl=\hul\,\ul$ must be positive in
all active reactions. Also note that external metabolites have an
economic potential $\wtoti=0$ unless the metabolite concentrations are fixed
by constraints or scored by the benefit function.  In a third
scenario, we introduce additional constraints (e.g.~upper or lower
bounds on fluxes).  \co{einzeln erklaren: or we assume benefit terms
  that score individual fluxes \co{irrespective of net metabolite
    production.}}  The corresponding Lagrange multiplier terms yield
{\fluxgain}s $\bvdirl$ which can replace the values $\wtotl$ from the
previous formula.  It can be practical to use formulae without any
{\fluxgain}s (because then the {\fluxvalue}s are given directly by
the economic potential differences). Formally, the {\fluxgain}s of
reactions with external reactants can be included in the external
economic potentials; and for reactions without external reactants, we
can introduce virtual external reactants whose economic potentials
represent the {\fluxgain}s.  \co{discuss flux bounds; lagrange mult
  for active constraints; signs from kuhn-tucker (kommt schon in
  haupttext vor; hierhertun?)}


\myparagraph{Enzyme-optimal states and economical {\flow}s}
\label{sec:derivationfromMCA}
The {\fluxbenefitbalance} Eq.~(\ref{eq:reactionbalanceeq}) holds for
all kinetic models in enzyme-optimal states \cite{lieb:14a}. If it can
be satisfied for a given {\flow}, we know that the {\flow} is beneficial
(i.e.~with a positive net benefit) and economical (i.e.~all enzymes
contribute to this benefit). This also means that the {\flow} can be
realised by a kinetic model in an enzyme-optimal state.  In metabolic
economics, the stationary fluxes $\vv$ and concentrations $\cv$ are
scored by a {\metabolicobjective} function
$\gplus(\uv) = \bbenefit(\vv(\uv),\cv(\uv))$, while the enzyme levels
$\ul$ are penalised by an enzyme {{\investment}} function
$\hminus(\uv)$. By choosing the enzyme profile with the maximal
fitness $\ffit(\uv)=\gplus(\uv)-\hminus(\uv)$, we obtain an
enzyme-optimal state. In this state, we define the {\fluxgain} vector
$\bvtot = \partial z/\partial \vv$ and the {{\enzymecost}}s
$\hudotl= \partial \hminus/\partial \ln \ul$ (i.e.~the
{{\enzymeprice}}s $\hul=\partial \hminus/\partial \ul$, multiplied
with the enzyme concentrations $\ul$). After omitting all inactive
reactions from the model, all reactions must have positive
{{\enzymecost}}s in order to satisfy the balance condition
$\partial \gplus/\partial \ul = \partial \hminus/\partial \ul$, and
the {\summationcondition}
\begin{eqnarray}
 \label{eq:fitnessbalance2}
 \bvtot\trans\, \delta \vv &=& {\vv\inv}\trans\, \diag(\hudot)\, \delta \vv,
\end{eqnarray}
must be satisfied by any stationary flux vector $\delta \vv$ (i.e.~any
vector satisfying $\Nint\,\delta \vv=0$). Here we assume that all
reactions are catalysed by specific enzymes; multifunctional enzymes
and non-enzymatic reactions require some changes in the formulae
\cite{lieb:14a}.  {\Flow}s satisfying the condition are called
\emph{economical}: they are free of {\nonbeneficial} modes \cite{lieb:14a}
and also satisfy the {\fluxbenefitbalance}
(\ref{eq:reactionbalanceeq}). \coout{The {\fluxbenefitbalance} itself
  is derived as follows: as an optimality condition, we obtain the
  equation $\v_{l}\gvtotl=\hudotl$ with the total {\fluxvalue}
  $\gvtotl$. The latter, in turn, can be rewritten as the flux
  {\myvalue} $\Deltar \wtotl + \bvdirl$, where the internal economic
  potentials are defined by the control coefficients of the metabolic
  objective function with respect to small virtual exchange fluxes of
  the metabolites.} This holds, for example, for {\flow}s obtained by
FCM.  Economical {\flow}s can be realised by various kinetic models with
different combinations of kinetic constants, {\metabolicobjective}s, and
{{\investment}} functions \cite{lieb:14a}.  \coout{Importantly, the
  concentration {\gain}s $\bcm$ do not appear in the
  {\fluxbenefitbalance} and can therefore be ignored here.}
Uneconomical {\flow}s, in contrast, cannot appear in any enzyme-optimal
kinetic model, and we may decide to discard them in flux analysis.

\myparagraph{Economic FBA} \co{der abschnitt ist schoen, aber im
  artikel nicht wirklich noetig .. eher als kurzbeschreibung
  anderswo?}  Economic FBA is a variant of FBA that uses the economic
potentials as free variables, like a second type of chemical
potentials. By employing the {\fluxbenefitbalance} as an extra
constraint, it ensures that the predicted {\flow}s can satisfy the
optimality conditions in flux minimisation or enzyme-optimal kinetic
models, and by doing so it unifies enzyme optimisation and flux cost
minimisation.  Enzyme optimisation in kinetic models (considering all
possible choices of rate laws and enzyme {{\investment}} functions)
and flux cost minimisation (considering all possible choices of flux
cost weights) have as solutions the set of economic metablic {\flow}s.
From a geometrical point of view, the flux benefit principle defines a
set of economically feasible segments in flux space (see Figure
\ref{fig:fbacomparison2}); intersecting them with the FBA-feasible
flux polytope $\fbaPolytope$ yields a collection of convex polytopes
of economical {\flow}s, each corresponding to a specific flux
pattern. The possible solutions of FCM lie in this polytope and fill
it completely.

\begin{figure*}[t!]
 \begin{center}
  \includegraphics[width=16cm]{\psfilesfluxes/fbacomparison.eps}
  \caption{Flux balance analysis constrains fluxes
    by stationarity, thermodynamic constraints, and economic
    constraints. (a) Example network (internal metabolites in box,
    fluxes shown as arrows). The production of B is assumed to be
    beneficial and the rate of the reaction A $\rightarrow$ X has an
    upper bound. The flux cycle between X and B and the {\nonbeneficial} flux
    between C and D do not contribute any benefit. In FBA, these
    fluxes are irrelevant for the metabolic objective and therefore
    remain undetermined. (b) In thermodynamic FBA, the flux cycle is
    supressed because it cannot be driven by chemical potential
    differences. (c) Flux minimisation excludes the pathway from X to
    B because it is longer and therefore assumed to be costlier, and
    it suppresses the flux C $\rightarrow$ D. (d) The flux benefit
    principle excludes the cycle flux and the flux C $\rightarrow$ D
    because they are \nonbeneficial. The two routes from X to B are feasible,
    and the choice between them depends on model parameters.}
  \label{fig:fbacomparison}
 \end{center}
\end{figure*}

\myparagraph{Overview of constraints used in flux prediction}
\label{sec:methodscomparison}
\coout{TOPIC: Which flux predictions will we obtain from the economic
  flux principle, and how do they compare to other methods? How does
  economic FBA compare to other flux prediction methods?}  Figure
\ref{fig:fbacomparison} shows different criteria for feasible fluxes
that are typically used to predict fluxes. Classical FBA (a) excludes
any flux cycles that unnecessarily decrease the yield by consuming
metabolic resources. Fluxes that do not affect the yield -- e.g.~the
cyclic submode between X and B, or the flux from C to D -- remain
undetermined and must be removed by further constraints.  Such
constraints can be derived from general principles, as implemented in
other methods. Thermodynamic constraints (b) can exclude flux cycles
because the cylces do not dissipate any Gibbs energy; the flux from C
to D remains undetermined because it may dissipate Gibbs free energy.
Economic constraints discard all fluxes that do not contribute to the
benefit, as expressed by the {\fluxbenefitbalance}.  In contrast to
FCM (c), where uneconomical fluxes just happen to disappear during
optimisation, economic FBA (d) excludes these fluxes by explicit
constraints. The same constraints can also be used in flux sampling
\cite{prsp:04} to restrict the solutions to economical {\flow}s. In
Figure \ref{fig:fbacomparison}, both fluxes between X and B -- and any
positive linear combinations of them -- are allowed; to select
plausible {\flow}s, some extra heuristics can be employed. While the
principle of minimal fluxes selects the shortest pathway, FCM may
favour any of the pathways or even convex combination of pathway
fluxes. The choice depends on the flux cost weights assumed. Thus, FCM
makes additional assumptions as compared to economic FBA. Instead of a
feasible {\fluxpattern}s, from which we can sample economical
metabolic {\flow}s, we obtain a single optimal {\flow}.


\subsection{Catalytic rates determine  embodied values and metabolic strategies}
\label{sec:SIchoiceMetabolicStrategies}

\co{den ganzen abschnitt in einen anderen artikel? zB FCM changes? CBA
  lagrange? CBA labour?} \co{sagen: wir sehen also, wie deie begriffe
  von ME es uns erlauben, intuitive ueberlegeungen zu metab strategien
  anzustellen, und dass diese ueberlegungen uebereinstimmen mit den
  vorhersagen herkoemmlicher modelle} We saw that the choice between
overflow metabolism and respiration can depend on enzyme investments
embodied in internal metabolites.  This prediction is in line with
existing arguments about rate-yield trade-offs \cite{wnfb:18}. For
example, it has been claimed \co{REF; montero?}  that high-yield
pathways show low rates (or, more precisely, show a high enzyme demand
per flux) because their low thermodynamic forces make the enzymes work
inefficiently, and the resulting lower flux (per enzyme molecule) must
be compensated by higher enzyme levels. By this argument,
substrate-efficient (high-yield) pathways would be generally
enzyme-inefficient (implying a lower growth rate), and this certainly
holds for strategies with very high yields, when the system encounters
severe thermodynamic bottlenecks (i.e.~some reactions are almost in
chemical equilibrium). \co{but not generally!}  To rephrase this
argument based on embodied costs, we note that higher driving forces
allow for lower {\enzymeinvestment}s at the same flux benefit. \co{leichte
  wiederholung mit abschnitt 3?}  Generally, the costs of an enzyme is
given by $\zcostgenerics = \Deltar \wtots \,v$ with a flux
$v = v_{+}\,(1-\e^{\Deltar G/RT})$, where $v_{+}$ is the forward
one-way flux and $(1-\e^{\Deltar G/RT})$ is the thermodynamic
efficiency factor \cite{nflb:13}.  Compared to a (hypothetical) fully
forward-driven reaction, the catalytic rate is decreased by a factor
$(1-\e^{\Deltar G/RT})$, and so the {\enzymeinvestment} per flux is
increased by a factor $ 1/(1-\e^{\Deltar G/RT})$.  Therefore, a
thermodynamic bottleneck in a pathway leads to higher embodied values
in all downstream metabolites.

This means, if a high-yield strategy leads to smaller driving forces
(everything else being equal), the metabolites will have higher
embodied values, \co{REST DES abschnitts kuerzen / nach SI?} and the
cell will favour yield-efficient metabolic strategies. To see this
more clearly, we note that the total {\enzymeinvestment} and enzyme
{\benefitshade}s in a pathway must be equal, as described by the
pathway balance equation (\ref{eq:PathwayBalanceEquation}).  In this
balance, by making the enzyme less efficient (e.g.~by smaller
thermodynamic forces $\theta_{l}$ or by a smaller external glucose
concentration decreasing $\eta^{\rm kin}$), \co{die zwei effekte
  sollten schon fruehzeitig im artikel klarwerden} we would increase
the cost on the right. If the economic potential on the left remains
constant, the yield on the left must increase. \co{this is, again, the
  short explanation of what's shown in the figure!}  \co{klarer sagen,
  dass die analyse hier eigentlich die lagrange-multiplikatore in
  stefans analyse betrifft!  .. and shows them from a different angle}

\subsection{Reasons for using economic balance equations}

FCM and economic FBA are almost equivalent in their assumptions and
predictions\footnote{Similar arguments can also be made for other
  methods, e.g.~FBA with molecular crowding, but for simplicity I
  shall only refer to FCM.}. Both methods trade flux benefits against
{\enzymeinvestment}s and predict that {\flow}s must be economical. FCM is
numerically cheaper than economic FBA, which requires mixed-integer
programming or enumerating all flux cycles.  So why don't we always
use linear FCM?  Economic FBA provides some new possibilities, for
example flux sampling under economic constraints, or the calculation
of economic potentials, which can be used to construct kinetic models
in enzyme-optimal states.  But the main advantage of economic FBA is
that it provides new theroretical insights.

\begin{enumerate}[leftmargin=5mm]
\item \textbf{General laws instead of case-by-case solutions} While
  FCM allows us to compute fluxes numerically, it does not explain,
  e.g.~why certain flux cycles are always suppressed.  Economic FBA
  can be used in both ways: to compute specific economical {\flow}s,
  or to characterise the set of economical {\flow}s as a whole. In
  theory, we might also explore this set by repeatedly running linear
  FCM with randomly chosen flux cost weights. Studying not only one
  economical {\flow}, but all of them, can clarify the mathematical
  relations between {\enzymeinvestment}s, flux {{\myvalue}}s, and the
  choice of economical fluxes.  Based on algebraic relations, we can
  detect and remove futile cycles; we can pinpoint how kinetics makes
  specific reactions or pathways profitable; and we can better
  understand the interplay between thermodynamics and optimality,
  reflected in the relationships between chemical and economic
  potentials.
  
\item \textbf{Connection to kinetic models} \co{etwas redundant} The flux cost functions in FCM
  can either be  defined ad hoc, without reference to
  specific kinetic models, or they can represent
  enzymatic or kinetic flux costs, as defined and computed
  in an underlying kinetic
  model. Similarly, economic FBA can employ  kinetic knowledge,
  e.g.~about enzyme efficiencies or {\enzymeinvestment}s, and the resulting
  economic potentials and {\enzymeinvestment}s can then be inserted into
  kinetic models. Knowing how to relate  {\enzymeinvestment}s (in kinetic
  models) to enzymatic flux costs (in flux analysis) also yields  a
  better understanding of flux cost functions in FCM.
  
\item \textbf{Justification for FCM} Economic FBA provides a
  theoretical justification for FCM.  Since economic FBA, FCM, and
  enzyme optimisation in kinetic models are equivalent, we know that
  the basic premise of flux cost minisation (the idea that fluxes, not
  enzymes, are costly) is not just a dogma, but reflects a truth in
  kinetic models! Moreover, economic FBA links the parameters of FCM
  (e.g.~linear flux cost weights) to biochemically meaningful
  quantities (enzyme and metabolite costs, enzyme kinetics, and
  metabolite concentrations) that are otherwise hidden in FCM.

  
\item \textbf{Enzyme {\investment}s appear as terms in the formulae}
  \co{das hier laeuft doch darauf raus, welche informationen man aus
    dem proteom herleiten kann; zb fluesse, wertfluesse, oder
    oekonomische potentiale. wo wird das hier behandelt? bei
    schaetzung von wertfluessen?  bei proteomaps in diskussion? bei
    schaetzung von fluessen aus enzymkosten (kommt am ende dieses
    abschitts)} Certain variants of FBA can use enzyme data and enzyme
  constraints in heuristical ways, for example, to define flux bounds
  proportional to the enzyme levels or to put constraints on some
  weighted sums of fluxes, as a linear proxy for enzyme amounts. The
  underlying assumption is that the enzyme efficiencies (i.e.~the
  fluxes per enzyme level) are constant and known. To translate fluxes
  into enzyme levels, we may divide them by the catalytic constant
  (assuming that enzymes work at full speed) or by the catalytic rate
  (accounting for incomplete capacity use due to physiological
  metabolite concentrations). The latter leads to higher enzyme
  demands).  \co{REF naama; ecm; fcm; determining the catalytic rates
    is difficult because they depend on metabolite concentrations,
    which are unknown and variable, and computing them by ECM would
    bring us back to enzymatic flux cost functions.} In FCM, \co{WO?
    we can use flux cost functions that represent the
    {\enzymeinvestment}s in kinetic models \cite{lieb:18fcm}, but
    these functions are nonlinear and hard to compute.} enzyme levels
  are usually linked to fluxes, e.g.~to define flux constraints.
  Economic FBA uses enzyme data in a different way: enzyme levels are
  directly associated with costs, which provide information about flux
  benefits.  The cost term in the economic balance equation represents
  {\enzymeinvestment}s, as defined in kinetic models, and can
  incorporate knowledge about enzyme levels, {\enzymeprice}s, or
  enzyme efficiencies into the model.  \co{criticism: letztlich eher
    schwacher vorteil, da die effizienzen doch wieder eine rolle
    spielen.  if {\enzymeprice}s and enzyme efficiencies are known,
    they can also be incorporated into FBA, e.g. FBA with molecular
    crowding. so where is the advantage?  difference: in eco FBA,
    knowledge about enzyme properties is not used to determine the
    fluxes, but the economic potentials!}

\item  \textbf{Inference of metabolic fluxes from known {\enzymeinvestment}s}
  \co{mit vorigem verbinden} If we claim  that a cell is  in an optimal
  state (i.e.~that the fluxes are economical), known {\enzymeinvestment}s
  $\zcostgenericl$ can be used to infer the metabolic fluxes. However,
  this works only if the {\enzymeinvestment}s and {\fluxgain}s are precisely
  known. The calculation  is based on the {\summationcondition} and
  explained in SI \ref{sec:fluxesfromenzymecosts} in \cite{lieb:14a}.
  \co{ref to Eq about lower limit} The given {\enzymeinvestment}s will
  determine the set of active fluxes, and from condition
  (\ref{eq:fitnessbalance2}), together with the stationarity
  condition, the fluxes and economic potentials $\wintm$ can be
  computed numerically (see \cite{lieb:14a} for examples). \co{NACH
    CBA I?:} Since the flux directions are not predefined in this
  case, there is no guarantee that the predicted fluxes will be  thermodynamically feasible.
  \coout{An example is shown in Figure \ref{fig:branchflux} in the
    SI.}

\item \textbf{Metabolite costs are hidden in the choice of fluxes and
    economic potentials} Economic FBA shows that flux costs can
  reflect not only enzyme costs, but also metabolite costs.  In
  chemical reactions, a higher substrate level increases the flux per
  enzyme, and therefore the catalytic rate. \co{die beispiele hier mit
    cba OPT und anderen artikeln abstimmen; tepper zitieren? density
    constraints for metabolites!} But it also increases osmolarity, it
  can increase metabolite loss by membrane leakage or dilution
  \cite{sche:91}, and metabolites can be toxic at higher
  concentrations. \co{mention metablite cost term in optimality
    principles} This trade-off between the benefits and costs of
  higher metabolite concentrations may affects the choice of optimal fluxes,
  and an economic theory of metabolism should be able to capture
  this. So how can we justify a method like FCM which ignores
  metabolite concentrations completely?  We have seen that whenever a kinetic
  model (accounting for metabolite costs) predicts an optimal
  metabolic state, there will also be FCM models (with corresponding
  flux cost functions) and economic FBA problems (with corresponding
  economic potentials) that predict the same fluxes! This shows that
  metabolite costs, no matter how they arise, can always be mimicked
  by flux cost functions and economic potentials. \co{interessant
    wirds es, wenn sich das konkretisieren laesst} But how fo these
  hidden metabolite costs translate into flux costs? In FCM, we can
  use kinetic flux cost functions which refer to a given kinetic model
  and, by definition, account for metabolite costs. By linearising
  this cost function, we obtain linear flux cost weights that also,
  effectively, account for metabolite costs.  Economic FBA, is turn,
  can rely on each of these model approaches, and the economic
  potentials can also reflect metablite costs.  Thus, the only
  remaining question is how to \emph{choose} the flux cost functions,
  the flux cost weights, or the economic potentials by heuristic
  assumptions, to make them reflect \emph{realistic} states of a
  kinetic model with metabolite cost. \co{also say that only one sort
    of equations from kinetic models is used (the one related to
    metabolite production andfluxes); the other one (the one related
    to metabolite concentrations, and thus metabolite cost) is ignored, which
    is the reasons why there are many possible solutions for the
    economic potentials (which is perfectly justified as long as we do
    not know the underlying kinetic model.)}
\end{enumerate}



==> sec_flux_analysis_overview.tex <==
\iftoggle{bookversion}{}
{\section{Flux analysis and economic constraints}}

A cell can show various metabolic {\flow}s, each characterised by
different enzyme investments, product yields, usage of cofactors, and
thermodynamic forces in the reactions.  Flux analysis predicts
plausible {\flow}s based on network structure and physical and
physiological assumptions: it either delimits possible {\flow}s or
selects one of them.  In this section, I review some concepts  and
methods for flux analysis, including methods that employ thermodynamic
or economic constraints.

\iftoggle{bookversion}
{\section{Metabolic fluxes and thermodynamic constraints}}
{\subsection{Metabolic fluxes and thermodynamic constraints}}
\label{sec:metabolicmodels}

\myparagraph{\ \\Metabolic networks and metabolic {\flow}s} We start with
stationary flux distributions or ``flows'' (if their absolute scaling
is disregarded, they are also called flux modes).  A metabolic network
is defined by a stoichiometric matrix $\Ntot$, which can be split into
submatrices $\Nint$ (for internal metabolites with concentrations
$c_{i}$ described by differential equations) and $\Next$ (for external
metabolites with predefined concentrations $x_{j}$).  A {\flow} $\vv$
must satisfy the stationarity condition $\Nint\,\vv = 0$.  {\Flow}s with
no net metabolite production or consumption at all (satisfying
$\Ntot\, \vv = 0$) are called \emph{cyclic}, and {\flow}s with a zero
flux benefit, satisfying
$\Nobj \,\vv = {\bvtot\trans \choose \Ntot}\, \vv = 0$ are called
\emph{{\futile}}. The vector $\bvtot$ represents flux-specific
benefits and can either stem from a kinetic model or be predefined by
the modeller.  The kernel vectors of the stoichiometric matrices
$\Nint, \Ntot$, and $\Nobj$, called stationary, cyclic, and {\futile}
flows, are columns of the right-kernel matrices ${\Kint}$, $\Ktot$,
and $\Kobj$ (satisfying $\Nint \,\Kint=0$, $\Ntot \,\Ktot=0$, and
$\Nobj\,\Kobj=0$).  Cyclic flux modes do not dissipate any Gibbs free
energy, which makes them thermodynamically infeasible: in models with a
production objective, these modes will be {\futile} (see section
\ref{sec:proofEquiEnergEcon}).

\co{klar definiert?  "konform": (a "konform" zu b):
   gegeben b, muss a dasselbe vorzeichen haben oder null sein.\\
   Aber wie nennt man Beziehung zwischen a und b, wenn a und b überall
   da, wo beide ungleich null sind, die gleichen Vorzeichen haben?
   Stefan: wir nennen das wieder conformal (denke dir: zu einem
   dritten vektor c). siehe unser bioinformatics paper (attached).}

\myparagraph{Active reactions and elementary modes} The active
reactions in a {\flow} $\vv$, (i.e.~reactions with non-zero rates) form
its \emph{active region} (or support) $\mbox{supp}(\vv)$. If all
reactions in a {\flow} are active, the {\flow} $\vv$ is called
\emph{pervasive}.  The \emph{overlap} of two {\flow}s $\vvA$ and $\vvB$
consists of the reactions that are active in both of the {\flow}s. A {\flow}
$\vv$ is called \emph{elementary} if there is no {\flow} $\kv$ with a
smaller support $\mbox{supp}(\kv) \subset \mbox{supp}(\vv)$.
Elementary cyclic, elementary {\futile}, or elementary
{\nonbeneficial} modes are defined similarly. If two {\flow}s $\kv$ and
$\vv$ show the same flux directions in all non-zero reactions of
$\vv$, we write this as $\kv \sqsubseteq \vv$ ($\kv$ is
\emph{conformal} to $\vv$), and if two {\flow}s $\vv$ and $\kv$ show the
same flux directions on their entire overlap, we also call them
conformal. If $\kv$ is a cyclic {\flow} restricted to the active region
of $\vv$ and if $\vv$ and $\kv$ are conformal, it is called a
\emph{conformal test mode} of $\vv$, and we say that $\vv$
\emph{contains a flux mode} defined by the {\fluxpattern} of $\kv$).

\myparagraph{Flux balance analysis} The aim of flux balance analysis
is to predict plausible {\flow}s, i.e.~the usage of metabolic pathways,
in metabolic networks \cite{vapa:94b}. The possible {\flow}s are
constrained  by stationarity and by  flux bounds:
\begin{eqnarray}
 \label{eq:fbastationarity}
 &&\Nint\, \vv = 0 \nonumber\\
 &&\vv^{\rm min} \le \vv \le \vv^{\rm max}.
\end{eqnarray}
The bounds can represent known physiological flux directions, the
impossibility of certain fluxes due to the absence of substrate, or
maximal fluxes caused by bounds on enzyme levels, and known flux
directions may also stem from a previous thermodynamic or economic
analyses. The conditions (\ref{eq:fbastationarity}) define a convex
polytope in flux space, called \emph{flux polytope}. Given a linear
benefit function (with benefit weights in a vector $\bvtotweight$),
optimal {\flow}s $\vv$ can be determined by maximising
$\bvtotweight\cdot \vv$
under the constraints (\ref{eq:fbastationarity}). In a typical usage,
classical FBA maximises the biomass production rate at a limited
nutrient uptake. Since the predicted biomass production is
proportional to the bound on uptake rates, FBA effectively maximises
the yield (biomass production per nutrient influx)
\cite{scpf:08}. Therefore, classical FBA predicts yield-efficient
strategies, even when yield-inefficient strategies are more profitable
(leading to faster growth). Moreover, FBA cannot select between flux
solutions of equal yield (even if their enzyme costs in reality are
very different).  Other FBA methods overcome these problems by putting
a cost (or constraints) on a weighted sum of absolute fluxes. Due to
the trade-off between flux cost and biomass production, low-yield
solutions may become favourable. Different FBA variants combine costs
and benefits in different ways: FBA with molecular crowding
\cite{bvem:07} optimises the metabolic benefit while putting a bound
on the total enzyme level. Flux cost minimisation, in contrast,
assumes a fixed benefit and minimises the flux cost. In both cases,
numerical optimisation will lead to an optimal {\flow}, which depends on
the quantitative parameters assumed in the enzyme {{\investment}}
function. For instance, known catalytic constants and enzyme {\price}s
can be used to obtain realistic flux predictions \cite{horh:11}. In
these methods, cost and benefit need not be compared on a common scale
because one of them is varied while the other remains  fixed.


\myparagraph{Thermodynamic constraints} According to the second law of
thermodynamics, fluxes must dissipate Gibbs free energy and must have
the same sign as the thermodynamic force
$\theta_{l} = - \Deltar \mu_{l}/RT$, with a vector
$\Deltar \muv = {\Ntot}\trans \muv$ describing chemical potential
differences along the reactions. There are two variants of this
condition \cite{bbcq:04}. According to the strong thermodynamic
condition (``strictly feasible fluxes''), any positive force must lead
to a positive flux:
\begin{eqnarray}
 \label{eq:ebastrong}
\mu_{l}\ne 0 \;\Rightarrow\; \quad v_{l}\,\Deltar \mu_{l} <0.
\end{eqnarray}
According  to the weak condition (``feasible fluxes''), any positive flux requires a positive force:
\begin{eqnarray}
 \label{eq:ebaweak}
 v_{l}\ne 0 \;\Rightarrow\; v_{l}\,\Deltar \mu_{l} <0.
\end{eqnarray}
With this condition, fluxes can always vanish, e.g.~because there is
no catalysing enzyme.
Some \coout{(e.g.~Energy Balance Analysis \cite{belq:02}, TMFA)}
variants of FBA employ  constraints that exclude thermodynamically
infeasible {\flow}s. 
Usually, the weak sign condition is
usually used. To ensure feasible flux distributions, we can treat
fluxes $v_{l}$ and chemical potentials $\mu_{i}$ as model variables:
the sign constraint Eq.~(\ref{eq:ebaweak}), together with upper and
lower bounds for $\Deltar \muv$, read
\begin{eqnarray}
 \label{eq:eba2b}
 && v_{l}\ne 0 \;\Rightarrow\; 
- v_{l} \, \sum_{i} N_{il}\, \mu_{i} > 0 \nonumber\\
 &&\Deltar \mu^{\rm min}_{l} \le \sum_{i} N_{il}\, \mu_{i} \le \Deltar \mu^{\rm max}_{l}.
\end{eqnarray}
The same condition can also be expressed differently, with the
chemical potential differences $\Delta \mu_{l}$ as free variables:
\begin{eqnarray}
 \label{eq:eba2}
 && v_{l}\ne 0 \;\Rightarrow\; - v_{l}\,\Deltar \mu_{l} > 0 \nonumber\\
 &&\Deltar \mu^{\rm min}_{l} \le \Deltar \mu_{l} \le \Deltar \mu^{\rm max}_{l} \nonumber \\
 &&{\Ktot}\trans \Deltar \muv = 0,
\end{eqnarray}
where $\Ktot$ is a right-kernel matrix of $\Ntot$.  The Wegscheider
condition in the last equation ensures that the vector $\Deltar \muv$
can satisfy an equality $\Deltar \muv={\Ntot}\trans \muv$.

\myparagraph{Cyclic flux patterns are infeasible thermodynamically} Given
a {\flow} $\vv$, how can we tell whether there exists chemical potentials
$\mu_{i}$ that comply with the given flux directions?  Beard et
al.~have given an algebraic criterion, the absence of flux cycles
(Theorem 6.1 in \cite{bbcq:04}). To check if $\vv$ is thermodynamically
feasible, one compares its {\fluxpattern} to elementary cyclic flux
modes, called elementary flux cycles.  In the terminology of oriented
matroids, elementary flux cycles are the elementary cycles of the
oriented matroid $M^{*}$ associated with the nullspace of the
stoichiometric matrix $\Ntot$.  For our feasibility check, we use the
notion of sign-orthogonality: two flux vectors $\av$ and $\bv$ are
sign-orthogonal if either they do not overlap (i.e.~they do not share
any active reactions), or if they share some reactions with identical
signs ($\sign(a_{l}) = \sign(b_{l})$) and others with opposite signs
($\sign(a_{j}) = - \sign(b_{j})$). \coout{Beard calls it ``strictly
  feasible'' and ``simply feasible'' instead} The two types of
thermodynamic conditions (strong (\ref{eq:ebastrong}) or weak
(\ref{eq:ebaweak})), lead to different feasibility criteria. if we
impose the strong condition (\ref{eq:ebastrong}), there is a solution
$\muv$ if (and only if) $\vv$ is sign-orthogonal on any cyclic {\flow} in
the network. In other words, cyclic {\flow}s cannot be conformal with
$\vv$. If we impose the weak condition (\ref{eq:ebaweak}), there is a
similar criterion: $\vv$ must satisfy
\begin{eqnarray}
 \label{eq:ebamatroid}
 | \sign(\vv)\cdot \sign(\kv)| < |\sign(\kv)\cdot \sign(\kv)|
\end{eqnarray}
for any cycle {\flow} $\kv$ \cite{bbcq:04}. As a consequence, any cyclic
flux mode $\modevectorcyc$ within the active region of $\vv$
must be sign-orthogonal on $\vv$. Thus, enumerating and testing
elementary cyclic {\flow}s allows us to find all local constraint
violations in a given {\flow}.

\coout{\textbf{Description by oriented matroids} FROM Oriented matroid
  theory: {\flow}s and modes support of {\flow} "opposite" {\flow} (=flow ith
  oppotite sign) distinguish "direction" of a flux from "orientation"
  of the reaction the sign of a flux describes direction relative to
  orientation if, then equivalently ...  "signed circuits": elementary
  *-modes zero mode is not an elementary *-mode!  for each elem
  *-mode, there is also the opposite el *-mode if X has a support
  within Y, they are either equal or opposite weak elimination: seien
  X und Y NICHT opposite: sei element e positiv in X und negative in
  Y. dann gibt es ein Z, das e nicht enthält und das nur positive
  elemente aus X und Y und nur negative elemente aus X und Y enthält.}
\coout{ORIENTED MATROIDS. stefan mueller: oriented matroids ``the essence
  of linear programming'' Theorem Rockafellar (1969): every flux mode
  can be written as a sum of elementary flux modes with matching sign
  patterns (ie conformal to the first one); elementary vectors and
  conformal sums; "submode" sign(e) $\le$ sign(f) e conforms to f all
  elementary flux modes conforming to f}
% articles:
% http://www-m10.ma.tum.de/foswiki/pub/Lehrstuhl/PublikationenJRG/21_OrientedMatroids.pdf
% http://www.ams.org/samplings/feature-column/fcarc-oriented1
% books:
% A. Bachem and W. Kern. Linear Programming Duality: An Introduction to Oriented Matroids. Universitext. Springer-Verlag, 1992.
% Ziegler, Günter M., Lectures on Polytopes, Springer-Verlag, New York, 1994.

  
\subsection{Origin of the economic balance equation}
\label{sec:justification}

In economic FBA the {\fluxbenefitbalance} (\ref{eq:reactionbalanceeq})
is used as a postulate. But how can it be justified?  And what do the
economic potentials and enzyme costs mean precisely?  In fact,
Eq.~(\ref{eq:reactionbalanceeq}) can be separately derived from
different underlying optimality principles, leading to different
interpretations of economic potentials and enzyme costs.  Aside from
the two derivations described below, economic potentials and
{\fluxbenefitbalance}s can also be obtained from a variety of other
optimality principles with the help of Lagrange multipliers
\cite{lieb:18lagrange}.

\myparagraph{Economic potentials obtained from flux cost minimisation}
The first optimality principle is flux cost minimisation (FCM)
\cite{lieb:18fcm}, a generalised form of FBA with minimal fluxes
\cite{holz:04,holz:06}.  FCM considers stationary {\flow}s with a
predefined flux benefit and determines the {\flow} that minimises a
cost function $\acost(\vv)$. This function can be the sum of absolute
fluxes $\sum_{l} |v_{l}|$, a weighted sum of fluxes
$\sum_{l} \acostvlweight\,|v_{l}|$, \cite{holz:04,scks:07}, or some
nonlinear cost function such as the enzymatic flux cost
\cite{nfbd:16,wnfb:18}. The only restriction is that flux costs must
increase with increasing fluxes, in the respective direction
(i.e.~$\sign(\partial \acost/\partial v_l) = \sign(v_l)$ whenever
$v_l \ne 0$).  The stationarity condition in FCM (all internal
metabolites must be balanced) gives rise to Lagrange
multipliers. These Lagrange multipliers satisfy balance equations of
the form (\ref{eq:reactionbalanceeq}) without any direction flux
{\gain}s (assuming the FCM problem contains no flux bounds)
and can therefore be interpreted as internal economic potentials
\cite{lieb:18lagrange}, while external economic potentials are given
by the production gains $\bvtotl = \partial \fluxbene/\partial v_{l}$
while enzyme costs defined as
$\zcostgenericl \sim (\partial \acost/\partial v_l)\,v_l$.  The proof
in \cite{lieb:18lagrange} resembles the way in which the thermodynamic
flux constraint $\Deltar \mu \cdot \, v <0$ is derived from a
principle of minimal energy dissipation (see SI
\ref{sec:fluxMinimisationProofChemical}). This means: {\flow}s that
satisfy a {\fluxbenefitbalance} Eq.~(\ref{eq:reactionbalanceeq}), and
only those {\flow}s, can be obtained by flux cost minimization.

\myparagraph{Economic potentials obtained from kinetic models}
Alternatively, Eq.~(\ref{eq:reactionbalanceeq}) can be derived from a
principle of enzyme-optimal states in kinetic models. We assume that
enzyme levels $\ul$ are chosen to maximising the difference between a
{\metabolicobjective} $\gplus(\uv)$ and an enzyme {{\investment}}
$h(\uv)$. In an enzyme-optimal state, the derivatives
$\partial \gplus/\partial \ln u$ (``\enzymebenefit'') and
$\partial \hminus/\partial \ln u$ (``\enzymecost'') must be balanced
for any active reaction.  As shown in \cite{lieb:14a} and SI
\ref{sec:derivationfromMCA}, the {\enzymebenefit}s can be written as
$\partial \gplus/\partial \ln u = [\Deltar \wtots + \bvdirs]\, v$
where the economic potentials $\wtotl$ are defined as derivatives of
the {\metabolicobjective} function with respect to virtual supply fluxes. By
setting $\zcostgenerics = (\partial \hminus/\partial e)\,u$, we obtain
the {\fluxbenefitbalance} (\ref{eq:reactionbalanceeq}).  With this
interpretation, the {\fluxbenefitbalance} guarantees that a {\flow} is
not only beneficial as a whole, but that each enzyme is used
beneficially. A similar condition exists in thermodynamics, where a
{\flow} must not only dissipate Gibbs energy as a whole, but must do
so in each single reaction.  \coout{Here met syst behave economically
  or behave thermodynamically; locally and globally beneficial fluxes are
  analogous to Gibbs energies dissipated by systems both as a whole
  and in every single reaction.}  So we can conclude: if a {\flow}
does not satisfy the {\fluxbenefitbalance} equation, it cannot be realised by
any kinetic model in an enzyme-optimal state. In flux analysis, we
discard such {\flow}s. 


\coout{refer to karush-kuhn-ticker conditions (``Lagrange
  multipliers'' of known signs, and non-zero only where constraint is
  active)} \coout{Lagrange multipliers are are equivalent to the ones
  obtained from {\MCA} // proof in CBA I; for definitions, see
  \cite{lieb:14a}).}  \coout{also mention applications of the
  Lagrange-approach in FCM; ECM; {\MCA}}


==> sec_flux_analysis_thermo.tex <==
\section{Economic and thermodynamic flux constraints}
\label{sec:economicandthermodynamic}

\co{WO?

  The two types of ``forces'' $w_{\rm v}= \Deltar w +\bvdirs$ and
  $\theta = \Deltar \mu$ cannot be strictly dependent. We can see this
  by a simple thought experiment. In a given metabolic state, we
  modify the kinetics of one of the enzymes: introduce an allosteric
  inhibition, while increasing the enzyme's $\kcat$ value in such a
  way that the two effects cancel each other.  The steady-state fluxes
  and concentrations remain unchanged. However, the change in kinetics
  will change the control coefficients, and therefore the economic
  potential difference $\Deltar w$ will change. Since the chemical
  potential differences $\Delta \mu$ remain unchanged, the two types
  of potentials cannot be strictly dependent.

}


\co{WO?} \co{also mention ronan's principle?}  \co{Mmh ..koennte man eine
  aehnliche annahme (per heuristik) auch fuer oekonomische flux-force
  relationship machen?  was waere die begruendung in bezug auf
  one-way-fluesse?  werden reaktionsereignisse wahrscheinlicher, wenn
  sie nuetzilch sind? wie haengt das damit zusammen, dass man
  thermodynamik aus flusskostenprinzip herleiten kann?}

\co{WO? FN? say that feasible flux states can be found using
  ronan's variational principle, treating economic potentials
  (virtually) as negative chemical potentials. (different choices of
  extra vector yield different possible flux solutions)}

\begin{figure*}[t!]
  \begin{center} 
\parbox[t]{8cm}{
(a) Thermodynamic constraints\\[5mm]
\includegraphics[height=1.9cm]{\psfilesfluxes/values_thermodynamics_text.eps}
\begin{center}
\fbox{\parbox{7.5cm}{
{\color{red} Positive Gibbs free energy dissipation} 
\[-\Delta_{r} \mu \cdot v = T \,\sigma > 0\]
Sign constraint: $\mbox{sign}(v) = \mbox{sign}(-\Delta \mu)$}
}\\[5mm]
{\scriptsize \begin{tabular}{lllll}
 Objective & Energy dissipation & $-\Deltar \muv\trans \, \vv$ \\[1mm]
 Potential & Chemical pot.~$\frac{\partial G}{\partial n_{i}}$ & $\mu_{i} = \mu^\circ_{i} + RT \ln c_{i}$ \\[1mm]
 Types of {\flow}s & Exergonic & $-\Deltar \muv \cdot \vv >0$ \\
 & Cyclic  {\color{red}\Lightning}  & $-\Deltar \muv\cdot \, \vv =0$ \\
 & Endergonic  {\color{red}\Lightning} & $-\Deltar \muv\cdot \, \vv <0$ \\[1mm]
 Matrix condition & Non-productive & $\Ntot \, \vv = {\Next \choose \Nint} \, \vv=0$ \\[1mm]
 Sign constraint & Locally exergonic & $v_{l} \ne 0 \;\Rightarrow\; -\Deltar \mu_{l} \, v_{l} >0$ \\[1mm] 
 \end{tabular}}
\end{center}
\includegraphics[width=6.5cm]{\psfilesfluxes/thermodynamic_cycles.eps}
}
\parbox[t]{8cm}{
(b) Economic constraints\\[5mm]
\includegraphics[height=1.9cm]{\psfilesfluxes/values_economics_text.eps}
\begin{center}
\fbox{\parbox{7.5cm}{
{\color{blue} Positive enzyme benefit} 
\[-\Delta_{r} w \cdot v = \hudots > 0\]
Sign constraint: $\mbox{sign}(y) = \mbox{sign}(\Delta_{r} w)$}
}\\[5mm]
{\scriptsize
 \begin{tabular}{lllll}
 Objective & Flux benefit & $\bvtot \cdot \vv = ({\Next}\trans \bpsi + \bvdir) \trans \, \vv$ \\[1mm]
 Potential &  Economic pot. & $\wextj = \bpsij$; $\winti = \frac{\partial \gplus}{\partial \varphi_{i}}$ \\[1mm]
 Types of {\flow}s & Beneficial &$\bvtot \cdot \, \vv >0$ \\
  & Useless  {\color{red}\Lightning}&$\bvtot \cdot \, \vv =0$ \\
  & Wasteful  {\color{red}\Lightning} & $\bvtot \cdot \, \vv <0$ \\[1mm]
 Matrix condition & Useless& $\Nobj\, \vv = {\bvtot\trans \choose \Nint} \, \vv=0$ \\[1mm]
 Sign constraint & Economical & $v_{l} \ne 0 \;\Rightarrow\; [\Deltar \wintl + \bvdirl]\, v_{l} >0$\\[2mm]
 \end{tabular}}
\end{center}\ \\[5mm]
\includegraphics[width=3.8cm]{\psfilesfluxes/loopexample_b_prices.eps}
\includegraphics[width=3.8cm]{\psfilesfluxes/loopexample_c_prices.eps}
}
\caption{Thermodynamic and economic flux constraints resemble each
  other. Based on three aspects -- mass balance, energy balance, and
  economic benefit -- {\flow}s can be categorised into productive or
  cyclic; exergonic, cyclic, or endergonic; and beneficial,
  {\futile}, or \wasteful. (a) Thermodynamic
  constraints. Non-productive modes dissipate no Gibbs energy.  In
  models with production objective, they are {\futile}. Cyclic and
  endergonic {\flow}s are thermodynamically infeasible. (b) Economic
  constraints.  In economic flux balance analysis, globally feasible
  {\flow}s are called economical, and globally infeasible {\flow}s are
  called \nonbeneficial. Conditions for infeasible fluxes are marked by the
  {\color{red}\Lightning} symbol. The symbol $n_{i}$ denotes the mole
  number of substance $i$.}
    \label{fig:analogiesFBAEBAVBA1}
  \end{center}
\end{figure*}

\subsection{Comparison of economic and  thermodynamic constraints}

\myparagraph{\ \\Economic analysis resembles thermodynamic flux
  analysis} \co{sort} There is a close resemblance bteween
thermodynamic and economic flux constraints. In both cases, flux
directions are determined by ``forces'' defined by potential
differences. Even if thermodynamic and economic constraints have different
physical justifications, this makes them very similar mathematically
(see Figure \ref{fig:analogiesFBAEBAVBA1}).  The economic constraint
Eq.~(\ref{eq:reactionbalanceeq2}) and the thermodynamic constraint
Eq.~(\ref{eq:thermocondition}) have a similar form and can therefore
be treated with similar methods (see Table in Figure
\ref{fig:analogiesFBAEBAVBA1}). \co{WD mit direkr drueber!}  In both
cases, the flux directions are determined by ``forces'' ($\Deltar \mu$
or $\Deltar w + z$), but a flux may always vanish despite a non-zero
force. While the thermodynamic constraint follows from physical laws, the
economic constraint is specific to steady, enzyme-optimal metabolic
states.  The thermodynamic and economic constraints show various
differences (and so it makes sense to use them both simultaneously in
a model):
\begin{enumerate}[leftmargin=5mm]
\item \textbf{Different assumptions} The thermodynamic and economic
  constraints represent logically different assumptions about
  cells. The thermodynamic constraint Eq.~(\ref{eq:thermocondition})
  follows from physical laws and must hold for any chemical reaction,
  no matter if it exists in a test tube or in a living
  cell. Constraint violations are only acceptable in ``incomplete''
  models, for example if cofactors are ignored. \co{can be fixed by
    extra term (mentioned below)} The economic constraint, in
  contrast, is specific to cells or technical systems in which enzyme
  levels are optimised.  Moreover, the thermodynamic constraint holds
  always, while the economic {\fluxbenefitbalance} only applies to
  steady states.
\item \textbf{Chemical and economic potentials} An economic potential
  is not a molecule property, but a variable that describes the
  changing fitness {\myvalue} of a metabolite. Also chemical potentials
  are variable, but unlike economic potentials they depend very
  strongly on metabolite concentrations.
\item \textbf{Independent choices of external potentials} The chemical
  potentials $\mu_{i}$ depend on the metabolite concentrations and
  Gibbs free energies of formation while the economic potentials
  $\wtoti$ arise from a metabolic objective function defined by the
  modeller. The two types of potentials carry different
  information and can be independently chosen. For instance, if the
  metabolic objective is biomass production, we can assign an economic
  potential of 1 to biomass and zero potentials to all extracellular
  metabolites. The chemical potentials have  different
  values and constrain the fluxes in different ways.
\item \textbf{Direct {\fluxvalue}} If a reaction is directly scored
  by the {\metabolicobjective} function, its direct {\fluxvalue} $\bvdirl$
  appears as a term in the {\fluxbenefitbalance}. Usually, there is no
  corresponding term in the thermodynamic constraint.  However, models in
  which cofactors are omitted may require such terms in the thermodynamic
  constraint (\ref{eq:thermocondition}). And, on the contrary, a flux
  {\myvalue} term can also be omitted by reformulating the model and
  replacing it by the economic potential of a virtual external
  compound.
\item \textbf{Reason for local constraints} According to
  thermodynamics, Gibbs free energy must be dissipated in every
  reaction. The reason is that the total Gibbs energy of the chemical
  system can be split into Gibbs energies of metabolites, and that
  reactions convert these metabolites individually. The economic
  constraint, in contrast, represents the global influence of enzymes
  on the metabolic objective. This influence is mediated by various
  pathways, involves changes of the steady state, and is therefore
  non-local. Only by using a trick -- rewriting the control
  coefficients in terms of economic potentials -- we can represent the
  constraint as a local balance condition.
\item \textbf{Local flux cycles and {\nonbeneficial} modes} To dissipate
  Gibbs energy in every reaction, {\flow}s must be free of flux cycles,
  i.e.~they must satisfy condition (\ref{eq:ebamatroid}) for any
  cyclic {\flow} $\modevectorcyc$ (i.e.~any {\flow} that satisfies
  $\Ntot\, \modevectorcyc=0$).  The criterion for economical
  {\flow}s is similar, and it is instructive to compare the two
  conditions. Beard et al.~ \cite{bbcq:04} have given an algebraic
  criterion for thermodynamically feasible {\flow}s, i.e.~flows that can
  satify the weak thermodynamic condition
  $v_l \ne 0 \Rightarrow \sign(v_l) = \sign(-\Deltar \mu_l)$.  The
  economic criterion is also a ``weak'' criterion: positive fluxes
  require positive {\fluxvalue}s, but a positive {\fluxvalue} does
  not imply a positive flux. \co{leichte wiederholung mit oben?} To
  formulate their criterion, Beard et al.~ compared the flux profile
  $\vv$ to elementary flux cycles, i.e.~elementary cyclic {\flow}s
  $\modevectorcyc$ satisfying $\Ntot\,\modevectorcyc=0$.
  If a {\flow} $\vv$ satisfies the weak thermodynamic condition, then all
  such modes $\modevectorcyc$ must satisfy
  $|\langle \modevectorcyc, \sign(\vv)\rangle| < |\langle
  \modevectorcyc, \modevectorcyc\rangle|$ (Equation 5.2
  in \cite{bbcq:04}).  As an equivalent condition, there cannot be any
  elementary flux cycle $\modevectorcyc$ whose support is
  within the support of $\vv$ and conformal with $\vv$. The criterion
  for thermodynamic feasibility has the same form as our criterion for
  economical {\flow}s, but with three main differences: (i) Thermodynamic
  feasibility is tested using cyclic flux variations, while economic
  feasiblity is tested using {\nonbeneficial} flux variations. (ii) The
  criterion for economic feasibility includes not only {\futile} flux
  variations, but also \emph{\wasteful} flux variations, whereas Beard
  et al.~do not consider exergonic flux variations. (iii) The
  criterion for economical fluxes is a \emph{sufficient}
  criterion, while  Beard et al.~provide only a necessary criterion.

\end{enumerate}

\coout{
\begin{figure*}[t!]
 \begin{center}
  \begin{tabular}{lll}
   (a)&(b)\\
  \includegraphics[width=7.3cm]{\psfilesfluxes/ycm_pmf_model_construction_atp_prod_aerob_glucose_mu_cofactors.eps}&
  \includegraphics[width=7.3cm]{\psfilesfluxes/ycm_pmf_model_construction_atp_prod_aerob_glucose_w_cofactors.eps}\\
 \end{tabular}
\parbox{8cm}{(c)\\
\parbox{7cm}{\caption{\co{c, balken lieber hellblau} Model of yeast central metabolism (compare
    Figure \ref{fig:yeastpotentials} and \ref{fig:yeastfluxanalysis})
    with cofactors shown.  The model contains 57 reactions and 68
    metabolites, 47 of which are internal. (a) Chemical potentials
    shown in shades of red (dark: high; light: low). (b) Economic
    potentials (blue: high. light: low. pink: negative) determined
    from the {\fluxbenefitbalance} and with postulated {{\enzymecost}}s
    (with proteome data from \cite{nkcn:12}).}
  \label{fig:yeastpotentialssplit}}}
 \end{center}
\end{figure*}
}

\myparagraph{Can chemical and economic potentials be treated as
  separate variables?}  Economic FBA treats chemical and economic
potentials as separate variables, assuming that they are physically
independent. Is this a reasonable assumption?  Unlike the chemical
potentials, economic potentials do not directly depend on metabolite
concentrations\footnote{This is an interesting difference. Even though
  the chemical potentials are also derived from an ``objective'' (the
  system's total Gibbs free energy), there is an (approximative)
  formula that relates them to concentrations!}. If a change in model
parameters increases a metabolite concentration, the economic potential of
this metabolite may either increase or decrease depending on the case,
so there is no fixed relationship between these two
variables. \co{Proof where?} If we consider a given kinetic model, the
choices of chemical and economic potentials will of course be
interdependent.  However, this dependence depends on kinetic details,
and if the kinetic model is unknown, we cannot conclude any general
dependencies except for those established through flux
directions. Thus physically it makes sense to regard chemical and
economic potentials as independent variables.

\myparagraph{Given the thermodynamic and economic constraints, chemical
  and economic potentials are coupled by fluxes} The fluxes in
economic FBA must satisfy thermodynamic and economic constraints and this
leads to dependencies between chemical and economic potentials.  Since
fluxes run towards smaller chemical and larger economic potentials,
economic potentials and chemical potentials can be expected to be
anti-correlated. In particular, the potentials must satisfy the
condition
$v_{l} \ne 0 \Rightarrow (\bvdirl + \Deltar \wtotl) \cdot \mu_{l} \le
0$. By studying how both constraints interact, we can appreciate some
of the difficult regulation problems that cells need to solve.
\coout{We can see an example in Figure
  \ref{fig:yeastpotentialssplit}.}


\subsection{Thermodynamic laws derived from flux cost minimisation}
\label{sec:fluxMinimisationProofChemical}


\myparagraph{\ \\Thermodynamic constraints can be derived from a principle of
  minimial energy dissipation.} Since thermodynamic and economic
constraints follow from optimality principles of the smae form,
thermodynamic constraints can be formally treated as economic constraints.
What metabolic objective do we need to assume to make the chemical and
economic potentials (and therefore, thermodynamic and economic
constraints) coincide?  Rayleigh's dissipation function
$T\,\sigma = - \sum_{l} v_{l}\,\Deltar \mu_{l}$ describes heat
production in a chemical system (where $\sigma$ is the entropy
production per volume). Written as a flux objective, it reads
$\bbenefit(\vv) = - \muv_{\rm ext}\trans\, \Next \,\vv$, which defines
the {\fluxgain} vector $\bvtot = - \Next\,\trans\, \muv_{\rm ext}$,
and so the external economic potentials are given by the negative
chemical potentials (while the {\fluxgain}s vanish). Thus, to obtain
internal economic potentials that solve the economic balance equation,
we can simply use the negative chemical potentials of the internal
metabolites; the {{\enzymecost}}s $\hudotl$ will represent Rayleigh's
dissipation function $T\,\sigma_{l} = - v_{l}\,\Deltar \mu_{l}$ in
each reaction.  When treating the maximal dissipation of Gibbs energy
as a fitness objective, the thermodynamic and economic constraints will be
completely equivalent.

\myparagraph{Equivalence of thermodynamic and economic constraints in some
  cases} If we impose thermodynamic or economic constraints on a flux
distribution, but do not specify any of the chemical or economic
potentials, we obtain the thermodynamic or economic loop constraints
(excluding {\flow}s that cannot appear under any choice of
potential). Usually, thermodynamic and economic loop constraints constrain
fluxes in different ways.  However, in some models these constraints
may be coupled or even identical.  In models with production
objectives ($\bvdir=0$), economical metabolic {\flow}s are free of flux
cycles\footnote{The proof is simple: in models with production
  objective, all cyclic flux profiles are {\futile} (i.e.,
  $\Ntot\,\kv=0\;\Rightarrow\; \Nobj\,\kv=0$). Thus, any {\flow} with a
  flux cycle will also contain a {\nonbeneficial} submode and, in turn, any
  economical {\flow} -- a {\flow} without {\nonbeneficial} modes -- will be free of
  flux cycles.}.  Thus, if we eliminate all {\nonbeneficial} modes -- for
instance, by flux cost minimisation -- we automatically obtain {\flow}s
that are economically and thermodynamically feasible.  The opposite
conclusion -- thermodynamically feasible modes are economical -- holds for
models with the following properties (proof in SI
\ref{sec:proofEquiEnergEcon}): the objective depends on net
production; the network structure allows for beneficial {\flow}s; and for
stoichiometric reasonse, the external production rates must show the
same ratios in all steady states\footnote{Due to network structure in
  some models, the external production rates may show the same ratios
  in all steady states. A mathematical condition is that
  $\mbox{rank}(\Next\,\Kmat)=1$. This holds, for example, if a model
  has no more than two external metabolites or if a model produces a
  single product (e.g.~biomass in a whole-cell model) from a fixed
  composition of substrates and with a fixed composition of side
  products (e.g.~CO$_2$). Such fixed production ratios are enforced,
  for example, in mixed acid fermentation by a need to balance the
  reduction equivalents.  }.  In this case -- and if the chemical or
economic potentials can be freely chosen otherwise -- the thermodynamic
and economic constrains are equivalent and exclude the same flux
cycles.

\subsection{Thermodynamic cost terms in reversible reactions}
\label{sec:thermoCostTerms}

As visible from Eq.~(\ref{eq:fluxBurdenEfficiencyDetailed}), smaller
thermodynamic driving forces $\theta$ and lower catalytic rates
require additional enzyme investments for compensation and thereby the
increase the flux {\burden}s. However, we can also quantify the cost
of microscopic reverse fluxes more directly.  If we split the net
reaction flux into a difference of microscopic forward and reverse
fluxes $v=v^{+}-v^{-}$, and the enzyme level, accordingly, into a sum
$\esymbol = \esymbol^{+}+\esymbol^{-}$ (where
$\frac{v^{+}}{v^{-}}=\frac{\esymbol^{+}}{\esymbol^{-}}$), the reaction
balance equation reads
  \begin{eqnarray} [\Deltar \wintl + \bvtotl] (v^{+}-v^{-}) = \hus\,
    (\esymbol^{+}+\esymbol^{-}),
  \end{eqnarray}
  and hence
  \begin{eqnarray}
    [\Deltar \wintl + \bvtotl] v^{+} = [\hus\, \esymbol^{+}] + [\hus  \esymbol^{-} + [\Deltar \wintl + \bvtotl]  v^{-}]
  \end{eqnarray}
  where the first bracket term on the right is the ``ideal'' cost of
  the enzyme, assuming the reaction were completely forward-driven
  (but with the same net flux), and the second bracket term is the
  (inevitable) ``cost of reversibility''. In \fluxvalueform (for a
  reaction with positive net flux $v>0$), the balance equation can be
  written as
  \begin{eqnarray}
  [\Deltar \wintl + \bvtotl]  = \hus\,\esymbol^{+}/v^{+}  + \hus\,\esymbol^{+}/v^{+}  + [\Deltar \wintl + \bvtotl]  v^{-}/v^{+}
  \end{eqnarray}
  where the three terms on the right refer to the ideal {\fluxburden},
  the additioanl cost for (waste of) reverse enzyme, and the value
  loss due to reverse conversion, respectively. All three terms are
  positive.



==> sec_proofs_flux_analysis_cba.tex <==
\subsection{Thermodynamic and economic constraints can be redundant}
\label{sec:proofEquiEnergEcon}

\coout{Criterion for fixed ratios erwaehnen? (schon erwaehnt im text):
  $\mbox{Rank}(\Next\,\Kmat=0$.}  We consider a model with production
objective $\bbenefit(\vv)={\bpsi}\trans\,\Next\,\vv$ and assume that
its network structure allows only for a single stationary flux mode,
or for flux modes with identical external consumption or production
rates.  We further assume that no numerical values for the potentials
have been defined. In such models, thermodynamic and economic constraints
are redundant.  This can be shown in three steps:
\begin{enumerate}[leftmargin=5mm]
\item In models with a production objective, 
 cyclic {\flow}s  are {\futile}.\\
 \textbf{Proof:} A cyclic {\flow} $\vv$ (satisfying
 $\Ntot\,\vv={\Next \choose \Nint}\, \vv = 0$) satisfies
 $\Nobj\,\vv={{\bpsi}\trans \Next \choose \Nint} \,\vv=0$ and is
 therefore {\futile}.
\item In models with a production objective, {\flow}s with cyclic submodes are uneconomical.\\
  \textbf{Proof:} Thermodynamically infeasible fluxes contain cyclic
  flux cycles. A flux cycle in a {\flow} $\vv$ is defined by an cyclic
  submode $\gammav$ satisfying $\Ntot\,\gammav=0$. This cycle is
  {\futile}; as a flux variation, it defines a \nonbeneficial submode.
  Therefore, $\vv$ is not economical.
\item In models with a production objective, in which the network
  structure enforces external production and consumption rates with
  fixed proportions, {\futile}
  modes are cyclic. \\
  \textbf{Proof:} We can assume two things: (i)
  $\mbox{rank}(\Next)=1$, because the external production and
  consumption rates show fixed ratios across all steady states; (ii)
  for the given external economic potentials, there exists at least
  one beneficial {\flow}. Under these assumptions, a zero benefit implies vanishing
  production rates: in such systems, the
  equation ${\bpsi}\trans\Next\,\vv=0$ implies $\Next\,\vv= 0$
  ({\futile}), and accordingly, $\Nobj\,\vv=0$ implies
  $\Ntot\,\vv= 0$ (cyclic).  \coout{\item If a model has a flux
    objective, but not a pure production objective, the statements
    above hold only for {\flow}s in which direct {\fluxgain}s do not
    contribute to the benefit; for such modes a vanishing production
    still entails a vanishing benefit.}
\end{enumerate}
Altogether, any flux variation that is  a {\futile} mode will
also be cyclic. Therefore, all {\flow}s with {\futile} submodes will be
thermodynamically infeasible.

\subsection{A lower bound on  $|{\Delta} \mu_l| \cdot {\Delta} \wtotl$,
  Eq.~(\ref{eq:potentialProduct})}
 \label{sec:SIpotentialProductProof}

The product $|\Deltar \mu_l| \cdot \Deltar \wtotl$ in an enzymatic
reaction $l$ can be estimated  from the $\kcat$ value and from the
 {\price} $\hul$ of the enzyme. For the proof, we assume a positive flux and we write the rate
law in the separated form  \cite{nflb:13}
\begin{eqnarray}
\label{eq:SIfactorised}
v_l = u_l\, k^{\rm cat}_l\,(1-\e^{\Deltar \mu_l/RT})\,\eta^{\rm kin}_l(\cv).
\end{eqnarray}
  The kinetic efficiency $\eta^{\rm kin}$ is a number between
0 and 1 and depends on the reactant concentrations  \cite{nfbd:16}.
We now set
\begin{eqnarray}
\Deltar w_l = \hul \frac{u_l}{v_l} = \hul
\frac{1}{k^{\rm cat}_l} \frac{1}{1-\e^{\Deltar \mu_l/RT}}.
\frac{1}{\eta^{\rm kin}_l}.
\end{eqnarray}
Noting that $1-\e^{-x} < x$ for $x \ne 0$, we obtain the approximation 
\begin{eqnarray}
\Deltar w_l >
\frac{\hul}{k^{\rm cat}_l} \frac{1}{-\Deltar \mu_l/RT}.
\end{eqnarray}
Since the flux is positive, we know that $\Deltar \mu_l$ must be negative and thus
\begin{eqnarray}
|\Deltar \mu_l| \, \Deltar w_l  > \frac{\hul}{k^{\rm cat}_l} \, RT > \frac{\hul^{\rm min}}{k^{\rm cat}_l} \, RT
\end{eqnarray}
This means: low driving forces (which occur close to chemical
equilibrium) imply large economic potential differences and therefore
large enzyme costs per flux.


% --------------------------------------------------------

\subsection{A lower bound on {\fluxvalue}s and on economic potential
  differences}
\label{sec:ProofMinimalFluxDemand}

To allow for a non-zero flux, the {\fluxvalue} $\hvs=\hudots/v$ of a
reaction must exceed some lower bound, which depends on two enzyme
properties: on the estimated {{\enzymeprice}}s $\hus$ and on the
catalytic constant $k^{\rm cat}$.  The proof is as follows. For
factorised rate laws Eq.~(\ref{eq:SIfactorised}) \cite{nflb:13} (and
assuming a positive flux), we obtain
\begin{eqnarray}
\label{eq:FluxValueEq2}
\Deltar \wtots + \bvdirs   = \frac{\hus}{v/u} > \frac{\husmin}{{k^{\rm cat} \,(1-\e^{-\theta})}} >
\frac{\husmin}{k^{\rm cat}} = \hvsmin,
\end{eqnarray}
where $\hulmin$ is a lower estimate of the {{\enzymeprice}}.  The
catalytic rate $\ratelaw_{l} = v_l/u_l$ can be estimated from the
forward $k^{\rm cat}$ value and from the thermodynamic force
$\theta = -\Deltar \mu/RT$ (which determines the ratio between net
flux and partial forward flux \cite{beqi:07,nflb:13}).  With estimates
for these quantities, we can put tighter constraints on the flux
{{\myvalue}} $\Deltar \wtots + \bvdirs$ and on the economic potentials
$\wtots$. If $\husmin$ and $k^{\rm cat}$ are known, their ratio
$\hvs^{\rm min} = \husmin/k^{\rm cat}$ serves as a lower bound on
$\Deltar \wints + \bvdirs$.  Knowing all this, we can replace the
enzyme benefit principle (\ref{eq:reactionbalanceeq2}) by the stricter
condition
\begin{eqnarray}
 \label{eq:reactionbalanceeq2a}
[\Deltar \wtots + \bvdirs] \, v > \hudotsmin,
\end{eqnarray}
which must hold for all active enzymatic reactions.  The value of
${\hudotlmin}$ can be estimated from enzyme parameters.


==> sec_supplement_flux_analysis_cba.tex <==
\co{WO? WEG? 
  \includegraphics[width=4.cm]{\psfilesfluxes/cba_yeast_ccm_futile_cycles_hist_futile_cycles.eps}

  Size distribution of elementary {\nonbeneficial} submodes. Typical
  sizes (numbers of active reactions) range between 20 and 40.}

\co{WO? 

  refers to Fig 5
  
  \myparagraph{Economic potentials and degradation costs} \co{discuss
  case of negative economic potentials; weiter unten: what's the direction of the
  value flow?} Interestingly, the economic potential can also tell us
about  enzyme investments downstream of the
metabolite: the economic potential of our metabolite X can also we
written as $w_{\rm X} = w_{\rm P} - \frac{z_{x \rightarrow p}}{v}$,
the economic potential of end product P minus the sum of enzyme
investments needed to convert X into P, divided by the flux.  \co{if
  the substrate was a ``free gift'', the economic potentials are given
  by the enzyme investments divided by the flux.} For example, we can
think of a toxic metabolite X, which needs to be converted into an
extracellular waste product (with a zero value). The economic
potential of X must be given by the total {\enzymeinvestment} of the
detoxification pathway (including export proteins), divided by the
detoxification flux, and with a minus sign. \co{was lernen wir?}
\co{however, negatives potential heisst nicht direkt gift} \co{auch
  auf simple ccm beispiel in cba II verweisen?}  \co{2. general
  inference of economic values and {\valueflow}s // reference to
  abchnitt in CBA I zu inference of economic potentials from variation
  conditions // hier nur schematisches bild mit wachsenden pfeilen?
  oder lieber nur in CBA lagrange?}
}

\section{How metabolic fluxes are shaped by enzyme economy}
\label{sec:potentialsinnetworks}

\co{allgemein $\zcostgeneric$  in SI verwenden}

\subsection{The usage of enzymes or pathways}

Under what conditions should different enzymes or pathways be used by
a cell?  In an optimal state, the {\fluxvalue} of an active
enzymatic reaction must be balanced with the {\fluxburden}, i.e.~the
{{\enzymeinvestment}} per flux. This means, first, if two reactions (or
pathways) have the same overall stoichiometry, only one of them can be
active -- unless the {\fluxburden}s are identical, which (given the
different kinetics) is highly unlikely\footnote{In reality, the flux
  {\burden}s may still be quite similar, and so use both enzymes
  together will almost be optimal.} Second, the maximal catalytic rate
of an enzyme defines a lower bound on the {\fluxburden}. For an
enzyme to be active, its {\fluxvalue} must exceed than this minimal
{\fluxburden}, and a similar rule can be given for entire
pathways. Let us see this  in detail

\myparagraph{A balance equation for linear pathways} In metabolic
models, a linear metabolic pathway can described, effectively as a
single reaction.  For a consistent economic theory, it is therefore,
important that economic balances for reactions and pathways have the
same form. In fact, we can easily derive a single pathway balance
equation between the total {\enzymeinvestment} and the total flux benefit.
With a pathway flux $v_{\rm L}$ (identical for all reactions; but
different flux stoichiometries can be takein into account), the
balance equation Eq.~(\ref{eq:gedankenexpsum}) can be written as
\begin{eqnarray}
 \label{eq:gedankenexpsum2}
 \left[\sum_{l \in L} \Deltar \wintl + \sum_{l \in L} \bvdirl \right]
v_{\rm L} = h_{u,L}\,\ul,
\end{eqnarray}
with the total pathway enzyme level $\ul=\sum_{l \in L} \,\ul$ and
apparent pathway cost
$h_{\rm u,L} = (\sum_{l} \ul\, \hul)/(\sum_{l} \ul)$.  \co{hier fehlt
  noch erklaereung von bvL. lieber die einfache formel betonen}
Eq.~(\ref{eq:gedankenexpsum2}), written as
$\Deltar w_{\rm L}\,v_{\rm L} = h_{\rm \u_L}\,\u_{\rm L}$, resembles
the balance equation for single reactions.  \co{also define effective
  ``pathway flux burden''}

\myparagraph{Lower bound on the  {\myvalue}}
\label{sec:usageofpathways} 
In a kinetic model, each enzyme has a maximal activity $k^{\rm cat}$
and a minimal {\price} $\hulmin$ (the cost per amount of enzyme at
small expression levels). The ratio $\hulmin/k^{\rm cat}$ defines a
lower bound on the {\fluxburden} \cite{nfbd:16}.  If the flux
{\myvalue} of the reaction is lower, the reaction must be inactive. To see this, we consider
the  {\fluxbenefitbalance}
(\ref{eq:reactionbalanceeq}) in the form\footnote{Here we assume
  (without loss of generality) that  flux and {\fluxburden}
  $\hvl$ are positive, and consider the $\kcat$ value in forward
  direction.}
\begin{eqnarray}
 \label{eq:forceequation}
  \Deltar \wtotl + \bvdirl = \frac{\hul} {v_{l}/\ul} = \hvl.
\end{eqnarray}
The enzyme {\price} $\hul$ is bounded from below by some lower value
$\hulmin$, and the catalytic rate $v_{l}/\ul$ is always lower than the
catalytic constant $k^{\rm cat} = (v_{l}/\ul)^{\rm max}$ (for the flux
direction chosen). Therefore, the ratio in
Eq.~(\ref{eq:forceequation}) will always be larger than
$\hvlmin = \hulmin / k^{\rm cat}$, which defines a lower bound on the
{\fluxburden}\footnote{To calculate the {\fluxburden} $\hvl$, we may
  estimate $\ul/v_{l}$ from measured proteome and flux data, while
  {{\enzymeprice}}s $\hul$ can be estimated from enzyme chain lengths,
  catalytic constants, and life times \cite{horh:11} (see SI
  \ref{sec:potentaislfromenzymepar}) \cite{szad:10}.\coout{Values for
    a rough numerical estimate are an effective lifetime of 30 minutes
    (for growing \emph{E.~coli} cells)} Of course, $k^{\rm cat}$ is
  only an upper bound on $v_{l}/\ul$; for a closer approximation, we
  may account for reversibility and thermodynamic forces
  \cite{nflb:13}. A further correction method for $\hvl$, assuming an
  optimal state, is described in section
  \ref{sec:SIAlgConstraintFluxBurden}. Finally, we may also put upper
  bounds on the {\fluxvalue} from estimates on the maximal
  {{\enzymeprice}} and on estimated minimal enzyme
  efficiencies.}. Note that the bound is a lower approximation only:
even at higher {\fluxvalue}s, the reaction may stay inactive. A
similar argument holds also for pathways instead of reactions. In an
unbranched pathway with a production objective and with lower
{{\enzymeinvestment}}s $\hulmin$, we can sum over the {\fluxbenefitbalance}s
and obtain the pathway balance
\begin{eqnarray}
\label{eq:criticalbenefit}
\Deltar w_{\rm L} = \sum_{l \in L} \frac{\hul\,\ul}{v_{l}} \ge \sum_{l \in L} \frac{\hulmin}{k^{\rm cat}_{l}}.
\end{eqnarray}
If the flux
{\myvalue} $\Deltar w_{\rm L}$ is below this bound, the pathway flux
cannot be economical.

\myparagraph{Choices between enzymes or
  pathways} \label{sec:isoenzymesandisopathways}
Isoenzymes are enzymes that catalyse the same reaction and share the
same {\fluxvalue}.  \coout{WEG? {\myvalue}
  $\gvtot = \Deltar \wint + \bvtot$. By taking the ratio of both flux
  benefit balances, we obtain
\begin{eqnarray}
 \label{isoenzymes1}
 \frac{(\Deltar w+z_{\rm v})\,v_{1} }{(\Deltar w+z_{\rm v})\,v_{2} } = \frac{\hminus_{u_{1}}\,u_{1}}{h^{\rm u}_{2}\,u_{2}} \qquad 
\Rightarrow \qquad \frac{h^{\rm u}_{1}\,u_{1}}{v_{1}} = \frac{h^{\rm u}_{2}\,u_{2}}{v_{2}} \qquad \Rightarrow \qquad {\hvs}_{1} = {\hvs}_{2}.
\end{eqnarray}
} Therefore, if two isoenzymes are simultaneously active in an optimal
state, their {\fluxburden}s (i.e.~{{\enzymeinvestment}}s per flux) must be
equal. If we pick a model (with randomly chosen kinetic constants) and
optimise its enzyme levels, it is highly unlikely that isoenzymes will
satisfy such an equality (unless they are physically identical).  Only
one the enzymes will be expressed, the one with the lower {\price}.
Like for single reactions, the {\fluxvalue} can also be used to
predict the choice between pathways.  In a pathway L, we define the
total enzyme level $\u_{L} = \sum_l \,\ul$ and the apparent
{\enzymeprice} $h_{u_L} = \frac{\sum_l \hul\,\ul}{\sum_l \ul}$; the
total {\enzymeinvestment} can therefore be written as
$y_L = \sum_l \zcostgenerics_{l} = h_{u_L}\,\u_{L}$.  With the representative
pathway flux $v_L$, we then define the pathway {\fluxburden}
$a_{v_L} = \frac{y_L}{v_L} = \frac{h_{u_L}\,\ul}{v_L}$, the total
enzyme cost per unit flux \cite{bnlm:10}.  If two pathways show the
same net flux stoichiometries, they are called
\emph{isopathways}. \co{The fluxes $v_{L}$ must be comparable between
  pathways, that is, pathways with equal fluxes $v_{L_{1}}=v_{L_{2}}$
  must show the same net conversion.} If the metabolic objective does
not depend on concentrations or fluxes inside the pathways, both
isopathways have the same {\fluxvalue}. To be simultaneously active,
they need to to satisfy
\begin{eqnarray}
 \label{isoenzymes2}
 \frac{v_{1}}{v_{2}} = \frac{\sum_{l \in 1} \hul\, \ul} {\sum_{l \in 2} \hul\, \ul} \qquad 
 \Rightarrow \qquad \frac{v_{1}/u_{1}^{\rm tot}}{h^{\rm u,tot}_{1}} = \frac{v_{2}/u^{\rm tot}_{2}}{h^{\rm u,tot}_{2}}
 \qquad \Rightarrow \qquad {\hvs^{\rm tot}}_{1} = {\hvs^{\rm tot}}_{2}
\end{eqnarray}
where $u^{\rm tot}_{L}$ is the total protein level in pathway $L$,
exactly the same {\fluxburden}.  However in a given kinetic model, it
is very unlikely that two isopathways satisfy this condition just by
chance, unless they are fully identical. \co{Thus, one of them will
  have a lower {\price} and will be preferred.}


\subsection{How to compute  economic potentials from fluxes and flux
  {\gain}s}
\label{sec:SIscalingProperties}

\co{mention proportional scaling of potential differences in
  unbranched chain?}  If fluxes or metabolic objectives in a pathway
are changing, the economic potentials will be changing, too.  The
metabolic objective of a pathway is reflected by the {\fluxgain}s
and, equivalently, by the economic potentials at the pathway
boundaries.  If a pathway is perturbed, the metabolic state changes,
and the precise changes depend on all kinetic details. To obtain rules
of thumb for the changing economic potentials, we consider an
approximation. \co{According to Eq.~(\ref{eq:balancedinvestments6}),
  the internal economic potentials depend linearly on external
  economic potentials and on direct {\fluxvalue}s.}  If economic
potentials are computed with heuristic assumptions as explained in
section \ref{sec:princdistribinvestment}, then given the pathway
fluxes $\vv$ and {\fluxgain}s $\bvtot$ (assuming uniform
{{\enzymeinvestment}}s and using Eq.~(\ref{eq:balancedinvestments4Opt})), or
given the fluxes $\vv$ and (approximate) {{\enzymeinvestment}}s
${\hudot}^{\rm data}$ (using Eq.~(\ref{eq:balancedinvestments6})), the
internal economic potentials can be computed from the external
economic potentials. Assuming either given or uniform
{{\enzymeinvestment}}s, we can determine the internal economic potentials as
a function $\wint(\vv,\wext)$.  This formula shows how perturbations
of fluxes $\vv$ or {\fluxgain}s $\bvtotweight$ affect the internal
economic potentials. For example, if we scale the external variables
($\vv$ and $\wext$) by a factor $\xi$, the changes in the internal
potentials follow from simple scaling considerations.  \co{diskutiere
  verschiedene skalierungsmoeglichkeiten: nochmal klarer machen, was
  bei princ of fixed {{\enzymeprice}}s los ist; hat flussskalierung
  einen einfluss auf minimal {\fluxvalue} constraint?}  \co{In
  addition, we need to consider the constraint S29?? and whether this
  constraint can still be satisfied after our perturbation.}
According to Eqs (\ref{eq:balancedinvestments3}) and
(\ref{eq:balancedinvestments6}), the economic potentials $\winti$
scale proportionally with the {\fluxgain}s $\bvtot$, but are not
affected by flux scaling. The constraint
Eq.~(\ref{eq:balancedinvestments4}) is affected by a scaling
$\wint \rightarrow \xi\,\wint, \bvtot\rightarrow \xi\,\bvtot$, and
also by a scaling $\vv \rightarrow \xi\,\vv$. However, it remains
unchanged under a simultaneous inverse scaling
$\wint \rightarrow \xi\,\wint, \bvtot\rightarrow \xi\,\bvtot, \vv
\rightarrow \frac{1}{\xi}\,\vv$.  Taken together, a flux increase (at
constant {\fluxgain}s $\bvtot$) leaves all internal economic
potentials unchanged, while the {{\enzymeinvestment}}s increase
proportionally. In contrast, an increase of the flux gains $\bvtot$
(at a constant flux) makes both $\wint$ and the {{\enzymeinvestment}}s
increase proportionally. If we \emph{decrease} the flux or flux
{\gain}, the {\enzymeinvestment}s decrease until the solution hits
a constraint; in this case, the pathway flux is switched off,
even though the \todo{desired flux or {\fluxgain}} was still
positive!  \co{The same conclusions holds both for the principles of
  uniform cost, known cost, uniform {{\enzymeprice}}s, and known
  {{\enzymeprice}}s.}  \co{They also remain valid if we consider the
  entire metabolic network instead of a single pathway.}  From these
scaling relationships, we can also obtain sum rules similar to the
theorems of Metabolic Control Theory (see the derivations in
\cite{lieb:18lagrange}). \co{die summenregeln als formeln angeben}

\subsection{Should cells use combined metabolic strategies?}  
\label{sec:SIcombinationOrAlternative}

\co{interessant: der abschnitt liefert eine direkte verbindung
  zwischen metabolic economic und FCM; vieleicht ausdruecklich darauf
  eingehen?}  \co{textteile von hier in den artikel schieben (hinter
  ``Isoenzymes and isopathways'')? teilweise nach artikel, teilweise
  hier diskutieren, welche rechenmethoden tatsaechlich verwendet
  werden sollen} \co{move some parts to other articles?}  \co{hier
  roten faden klarkriegen. realitaet; formalismus; praktische
  vorgehensweise beim samplen?}

\myparagraph{\ \\Pure and combined strategies} A cell may accomplish
the same production task by different pathways (e.g.~it may use
fermentation or respiration to produce ATP at a given rate). Moreover,
these pathways may be used separately or in combination, i.e.~by a
linear supposition of pathway fluxes. Also isoenzymes could either be
used exclusively or in combination. In reality, often one pathway is
used at a time: for example, when bacteria grow on glucose, they often
repress the uptake of other carbon sources, even if these carbon
sources are available in the growth medium\footnote{The co-utilisation
  of glucose and malate in \emph{B.~subtilis} is a known exception.}.
\co{below: consider the case in which two pathways provide exactly the
  same net consumption and production (except for fitness-neutral
  differences, e.g.~usage of different ``cost-free'' nutrients.}  In
VBA this leads to the question: given our polytope of
economical {\flow}s (with pure pathway strategies on the boundaries,
and combined strategies inside the polytope), should we assume that
real metabolic {\flow}s can be anywhere in the polytope, or should we
rather assume that real {\flow}s must be sparse, and thus on polytope
vertices?  In the first case, it would make sense to sample solutions
from the entire polytope, whereas in the second case, we should pick
solutions only among polytope vertices.  Interestingly, this is also
what is most likely to happen in FCM (or in FBA with a minimal
weighted sum of fluxes), where due to the concave or linear flux cost
functions, the solutions are likely to lie on the boundary\footnote{If
  we consider alternative pathways in linear FCM, one of the pathways
  will be selected depending on the flux cost weights in the two
  pathways. Only if the two alternative pathways are completely
  identical (including the flux costs), a superposition of the two
  pathways is also allowed. However, if the flux cost weights were
  chosen at random, this case occurs with zero probability.}.
\co{mention relation to EFMs, cite EFM-FCM} Finally, we may also
envisage a third possibility: cells might combine as many strategies
as possible, and realise a very non-sparse flux distribution in the
centre of the polytope.  So, in Figure \ref{fig:fbacomparison2}, for
example, will the {\flow} shown by cells be located in the entire blue
triangle, on the dark blue edges, or in the triangle center?

\myparagraph{Arguments for pure strategies} The idea that
metabolic flux distributions should be sparse and that alternative
pathways should not be used in combination is supported by several
arguments. First, in flux cost minimisation the enzymatic flux cost is
a concave function on the flux polytope, so enzyme-optimal {\flow}s will
be located on vertices of the (benefit-restricted) flux polytope
\cite{wpht:14,murs:14}.  \co{lieber: samplen?  wenn optimum gewuenscht
  wird, In practice, lieber sparse!}  Exceptions can only occur if two
enzymes or pathways show exactly the same kinetics and cost functions
\cite{lieb:18fcm}.  Kinetic models in enzyme-optimal states lead to
the same conclusion: if alternative pathways are used simultaneously,
they are subject to the same economic potential difference, so they
must show the same enzyme cost. If we sample kinetic models (by
randomly assigning kinetic constants) and compute their enzyme-optimal
flows, it is very unlikely that alternative pathways will have exactly
the same flux costs.  According to these arguments, pathways should
not be combined, and isoenzymes and isopathways should be used
alternatively rather than in combination.

\myparagraph{Arguments for combined strategies} However, there are
also arguments for using combined {\flow}s. The most striking argument is
that such modes are observed in cells \co{ueberlagerung von el modes.
  zb warburgeffekt} How can we obtain combined strategies in models?
First, a superposition of basic {\flow}s may be enforced by constraints
(e.g.~when the maximal capacity of respiration is reached due to
crowding of respiratory chain complexes on cell membranes, additional
overflow may be required.  Second, there might be optimality reasons
(analogous to constraints) for adjusting the cell state in such a way
that isoenzymes show identical flux burdens. \co{compare to
  self-organised criticality} Third, some side objectives may be more
important than strict cost optimality. For example, nutrient
transporters with binding affinities are often expressed
simultaneously. This contradicts the idea of strict cost minimisation,
but it may provide an advantage when cells need to anticipate possible
changes in their environment (changing concentrations of the
nutrient). Even if a combined strategy is sub-optimal, the cost
disadvantage may not be large.  There are many such cases of
preemptive protein expression. \co{consider ``free'' benefit, similar
  to ``free energy in thermodynamics''; discuss this in FCM, cite it
  here} In this case, it would be unrealistic to expect that only the
nominally best state (with sparse fluxes) is actually reached. So the
actual question would be: if a ``pure'' strategy is better than
combined strategies, how big is the actual fitness difference?

\myparagraph{Consequences for flux sampling} This question -- whether
cells should use sparse or combined fluxes -- is important for flux
prediction by sampling.  If we sample parameter variants of a kinetic
model and compute the enzyme-optimal states, we will \emph{only}
obtain {\flow}s that are polytope vertices, just like in FCM.  However,
if we sample {\flow}s uniformly from a flux polytope, polytope vertices
will be sampled with probability 0.  So what should we do? If we trust
our previous argument -- especially the fact that optimal flux
distributions, according to FCM, are elementary modes
\cite{wpht:14,murs:14} -- a uniform flux sampling might be
unrealistic, and we should rather sample polytope vertices. Bu to
account for unknown circumstances (e.g.~preemptive expression),
sampling the entire polytope may be a better strategy. \co{it depends
  on what we want: if we want to sample POTENTIALLY optimal {\flow}s, the
  interior of the polytope can be discarded; if we sample uniformly to
  approximate a Boltzmann-sampling with flux cost as energy, this is
  OK}
  
  \co{Heuristic criteria for choosing between flux profiles exist, but
    they rely on details of kinetics and enzyme {{\investment}}
    function, which require additional assumptions like the assumption
    of uniform {{\enzymeinvestment}}s, or estimated flux costs.}  \co{The
    practical procedure involves a choice of fluxes PRIOR to the
    choice of economic potentials.}  \co{In any case, theory can help
    us see what follows from our (potentially limited or wrong)
    optimality assumptions.}
\co{4: PRACTICAL CHOICE: PICKING A REPRESENTATIVE, NON-SPARSE
  SOLUTION. Still, sampling or picking a single solution would be suggested by a
  principle of insufficient reason: without any additional knowledge,
  it would be implausible to pick one of the edges by chance. However,
  in doing so, we should keep in mind that the solution we pick does
  not only have zero probability, but that it is also worse than the
  best solution on the polytope surface.}

\co{WO? RUNTER ZU abschnitt ueber PFK/FBAsse (``Beispielmodelle'')?
  EXAMPLE: Economic balance in overflow metabolism (may rather in CBA labour?)

\begin{figure*}[t!]
 \begin{center}
 \includegraphics[width=8cm]{\psfilesfluxes/example_overflow_balance.eps}
 \caption{\co{WRITE ME}}
 \label{fig:overflowBalance}
 \end{center}
\end{figure*}

  [WRITE ME!]
  
  Transport - Glycolysis (2 ATP) - Overflow bzw TCA (18 ATP) two
  There are two elementary {\flow}s (fermentation + respiration)

  Consider mixed {\flow}s:

  $\vv = \sigma \,\vv_{\rm F} + (1-\sigma)\, \vv_{\rm R}$

  $\Delta w = 2\, \sigma \,w_{\rm ATP} + 20\, (1-\sigma)\, w_{\rm ATP} = (20-18\,\sigma) w_{\rm ATP}$

  Total flux benefit:

  $\Delta w \cdot v = z = z_{\rm trans} + \sigma \,y_{\rm F} + (1-\sigma)\, y_{\rm R}$

  \begin{eqnarray}
    \Delta w &=& a_{\rm trans} + \sigma \,a_{\rm F} + (1-\sigma)\, a_{\rm R} \\
             &\ge& a_{\rm trans} + \sigma \,a^{\rm min}_{\rm F} + (1-\sigma)\, a^{\rm min}_{\rm R}\\
             &=& a_{\rm trans} + a^{\rm min}_{\rm R} + \sigma\, (a^{\rm min}_{\rm F}-a^{\rm min}_{\rm R})
  \end{eqnarray}
  So altogether
  \begin{eqnarray}
    20 w_{\rm ATP}- a_{\rm trans} - a^{\rm min}_{\rm R} &=& \sigma \,(18 \,w_{\rm ATP} + a^{\rm min}_{\rm F}-a^{\rm min}_{\rm R}) \\
    \Rightarrow 
    \sigma  &=& \frac{20 w_{\rm ATP}- a_{\rm trans} - a^{\rm min}_{\rm R}}{(18 \,w_{\rm ATP} + a^{\rm min}_{\rm F}-a^{\rm min}_{\rm R})}                                                           
  \end{eqnarray}
  Critical $a_{\rm trans} = 20 \,w_{\rm ATP} - a^{\rm min}_{\rm R}$. Above this value, $\sigma =0$ and
  $20 \,w_{\rm ATP} = a_{\rm trans} + a_{\rm R}$, i.e. the ATP value increases.

}


\section{Algorithms for economic flux balance analysis}
\label{sec:algorithmsflux}

\subsection{How to calculate economical flux modes and economic potentials}

\coout{\ \\Computing economical fluxes and economic potentials in a
  network} According to the benefit principle, active enzymes in
enzyme-optimal states must have positive influences on the
{\metabolicobjective}.  This implies that the {\flow} $\vv$ must satisfy the
{\fluxbenefitbalance} Eq.~(\ref{eq:reactionbalanceeq}),
$[\Deltar w+ \bvdirs]v = \zcostgenerics$ with internal economic potentials
$\winti$ and positive {{\enzymeinvestment}}s $\zcostgenerics_{l}$.  To employ this
principle in FBA, we treat the economic potentials as variables and
impose the {\fluxbenefitbalance} as a constraint.  Given the flux
{\gain}s $\bvtotl$, we can then determine the stationary fluxes
$v_{l}$, chemical potentials $\mu_{i}$, and economical potentials
$\wintm$ by requiring stationarity, thermodynamic sign constraints, and
the {\fluxbenefitbalance} equation. In practice, solutions can be
found by mixed-integer linear programming. But this may be difficult,
and we can also compute the variables step by step:

\begin{enumerate}[leftmargin=5mm]
\item \textbf{Flux pattern}
  First, we determine a {\flow} with thermodynamically and
  economically feasible flux directions. Such {\flow}s can be obtained by
  flux cost minimisation. By running FCM with different choices of flux cost
  weights, we obtain {\flow}s with different {\fluxpattern}s.
  Alternatively, we can start from some uneconomical metabolic {\flow} and
  remove all flux cycles and {\nonbeneficial} modes (see
  \ref{sec:removefutilecycles}).
\item \textbf{FLow} Based on our feasible flux pattern, we can
  construct various {\flow}s with this \fluxpattern and with more
  realistic flux magnitudes. Such {\flow}s can be obtained by FBA or by
  flux sampling. \co{andere tricks?}
\item \textbf{Economic potentials and {{\enzymeinvestment}}s} Given the flux
  directions, we next determine chemical and economic potentials.  In
  the calculation, we use the {\fluxbenefitbalance} as a linear
  constraint and determine the economic potentials by linear
  optimisation or by sampling; the {{\enzymeinvestment}}s $\zcostgenerics_{l}$ follow
  automatically from the {\fluxbenefitbalance}.  The resulting fluxes
  and economic potentials will be formally feasible, but possibly
  unrealistic (i.e.~very different from the fluxes and economic
  potentials that would be obtained from realistic kinetic models).
  For example, if we sample the economic potentials, the resulting
  {\enzymeinvestment}s may imply very large {{\investment}}s in unimportant
  enzymes. To obtain realistic potentials, we may account for known
  enzyme properties such as molecular weights or catalytic constants,
  use other data, e.g. known or guessed fluxes and enzyme levels, or
  employ some heuristic assumptions (see sections
  \ref{sec:princdistribinvestment} and
  \ref{sec:potentaislfromenzymepar}).
\item \textbf{Constructing other solutions by varying a given
    solution} Once we have found a solution, we may vary it to
  generate other, more realistic solutions.  Starting from fluxes
  $\vv$ and economic potentials $\wint$, we may keep the economic
  potentials $\winti$ fixed, vary individual fluxes (where the fluxes
  need to remain stationary and flux signs are fixed), and vary all
  {{\enzymeinvestment}}s proportionally. Alternatively, we may fix the
  fluxes and vary the {\fluxvalue}s $\Deltar \wtotl + \bvdirl$ and
  costs $\zcostgenerics_{l}$ proportionally. Finally, in models with moiety
  conservation (e.g.~[ATP] + [ADP] = const), we may vary the economic
  potentials by adding an arbitrary conserved moiety vector
  $\mathfrak{g}$ (satisfying $\mathfrak{g}\trans \,\Ntot=0$) to
  $\wtot$. The potential differences $\Deltar \wtotl$
  (e.g.~$w_{\Deltar \rm ATP} = w_{\rm ATP}-w_{\rm ADP}-w_{\rm
    phosphate}$), {{\enzymeinvestment}}s, and enzyme benefits will not be
  affected by this.  Starting from a solution ($\vv, \wint, \hudot$)
  and varying it in these ways, we obtain an ensemble of possible
  solutions, or we can construct solutions that comply with other
  knowledge or data.
\end{enumerate}

\subsection{How to check flux modes for being economical}
\label{sec:appcriteria} 

\myparagraph{\ \\Criterion for economical metabolic {\flow}s} A {\flow}
$\vv$ is called economical if it satisfies the {\summationcondition}
Eq.~(\ref{eq:fitnessbalance2}).  Eq.~(\ref{eq:fitnessbalance2})
applies only to {\flow}s in which all reactions are active. By
definition, a {\flow} with inactive reactions economical if the same
flow, with all inactive reactions omitted, is
economical\footnote{Inactive reactions can be ignored and be removed
  from the model. To justify their vanishing fluxes, we can always
  assume large {{\enzymeprice}}s in the underlying kinetic
  model.}. Economical {\flow}s must satisfy the flux variation criterion
\cite{lieb:14a}, which compares an economical {\flow} $\vv$ to a test
mode $\modevector$ (i.e.~a stationary {\flow} on the active region of
$\vv$). For an economical {\flow}, the following holds: (i) If
$\modevector$ is beneficial ($\bvtot\cdot \modevector>0$), then $\vv$
and $\modevector$ must share some active reaction with the same flux
directions.  (ii) If $\modevector$ is {\wasteful}
($\bvtot\cdot \modevector<0$), then $\vv$ and $\modevector$ share some
reaction with the opposite flux directions. (iii) If $\modevector$ is
{\futile} ($\bvtot\cdot \modevector=0$), they must share both sorts
of reactions. This leads to the submode criterion: economical {\flow}s
must not contain any {\nonbeneficial} submodes\footnote{In a model with a
  production objective, this criterion shows that an economical flux
  profile is thermodynamically feasible: if there were an elementary flux
  cycle, indicating thermodynamic infeasibility, the {\flow} would be
  uneconomical.}. To apply this criterion, we only need to consider
elementary test modes. The submode criterion implies that economical
metabolic {\flow}s $\vv$ are beneficial (i.e.~have a positive total flux
benefit $\bvtot\cdot\,\vv$). To see this, we insert $\kv=\vv$ into the
{\summationcondition} Eq.~(\ref{eq:fitnessbalance2}) and obtain the
equality $\sum_{l} \zcostgenerics_{l} = \bvtot\cdot \vv$. Since the
{{\enzymeinvestment}}s $\zcostgenerics_{l}$ are positive, the benefit must also be
positive.

\myparagraph{Practical tests for economical {\flow}s} Constructing
feasible metabolic {\flow}s can be difficult because the thermodynamic and
economic flux constraints are nonlinear. The resulting mixed-integer
linear problems are numerically much harder than linear FBA. However,
checking a given {\flow} $\vv$ is relatively easy: it amounts to solving
linear satisfiability problems. There are several possibilities:
\begin{enumerate}[leftmargin=5mm]
\item \textbf{{\Summationcondition}.}  To satisfy the variation
  condition (\ref{eq:fitnessbalance2}), there must be {\fluxburden}s
  $\hvl$, with the same signs as the fluxes $\v_{l}$, satisfying
\begin{eqnarray}
 {\Kint}\trans \hvv &=& {\Kint}\trans \bvtot \nonumber \\
 \label{eq:signvectorcondition1}
 \diag(\vv)\, \hvv &>&0.
\end{eqnarray}
${\Kint}$ is a right-kernel matrix of $\Nint$ and its columns span the
space of stationary flux distributions.  The inequality ensures that
$\vv$ and $\hvv$ have the same sign patterns.

\item \textbf{{\Fluxbenefitbalance}: check the existence of
  consistent economic potentials.} An {\complete} {\flow} $\vv$ is
  economical if and only if it satisfies the benefit principle
\begin{eqnarray}
 \label{eq:signvectorcondition12}
 \diag(\vv)\, ({\Nint}\trans \wint + \bvtot) &>&0,
\end{eqnarray}
 with a  vector $\wint$ to be determined.  For  a practical test this, we search for 
 a difference vector $\Deltar \wint$ satisfying 
\begin{eqnarray}
 \label{eq:signvectorcondition13}
 \diag(\vv)\, (\Deltar \wint + \bvtot) &>&0 \nonumber\\
 {\Kint}\trans \,\Deltar \wint &=& 0.
\end{eqnarray}
The second line is a Wegscheider condition for $\Deltar \wint$,
ensuring that $\Deltar \wint = {\Nint}\trans \wint$ with some vector
$\wint$ \cite{wegs:02,scsc:89}.  Even if $\bvtot$ is not
known, we can constrain it by inequalities of the form
$\Qmat\, \bpsi > \qv$, which puts
 constraints on the flux directions. In this case, to show that a
flow $\vv$ is economical, we need to find a vector
${\bpsi \choose \hudot}$ such that
\begin{eqnarray}
 \label{eq:vbaconstraint2}
 {\Kint}\trans \left({\Next}\trans,\,-\diag(\vv)\inv\right) { \bpsi\choose \hudot} &=& 0 \nonumber\\
 \begin{pmatrix} \Qmat &0 \\0& \Imat\end{pmatrix} { \bpsi\choose \hudot} &>& {\qv \choose 0}.
\end{eqnarray}
\end{enumerate}
The criteria (\ref{eq:signvectorcondition1}) and
(\ref{eq:vbaconstraint2}) do not concern only  {\flow}s with inactive
reactions. Thus, to use this criterion, all inactive reactions must
first be removed from the model. Eqs (\ref{eq:signvectorcondition12})
and (\ref{eq:signvectorcondition13}), in contrast, apply directly to
the active reactions, while inactive reactions can be ignored (and 
their vanishing fluxes can be justified by assuming high
{{\enzymeprice}}s).

\subsection{How to eliminate thermodynamically or infeasible submodes} 
\label{sec:removefutilecycles} 

If no consistent chemical (or economic) potentials canbe found for a
given {\flow}, we know that this {\flow} is thermodynamically (or economically)
infeasible. But how can we localise the problem, i.e.~how can we
detect the problematic reactions or cycles, and how can we know which
fluxes need to be set to zero to obtain a feasible flux distribution?
Cyclic submodes (which violate thermodynamic laws) can be detected and
removed with the help of elementary flux modes.  Futile submodes
(which make a {\flow} uneconomical) can be treated similarly.  For
medium-sized networks, the elementary cyclic modes can be enumerated
by \emph{efmtool} \cite{efmtool} and be collected as columns in a
matrix $\Cmat$. Let $\vv$ be the {\flow} in which flux cycles should be
found and removed.  First, we reorient all reactions to avoid negative
fluxes.  Depending on the feasibility criterion we are interested in
(weak or strong thermodynamic feasibility, see SI
\ref{sec:metabolicmodels}, or economic feasibility), there are
different algorithms (see Figure \ref{fig:corrections}):

\begin{enumerate}[leftmargin=5mm]
\item \textbf{Respecting the strong thermodynamic condition} The strong thermodynamic
  flux condition states that non-zero driving forces cause non-zero
  fluxes in the same direction. To comply with such a condition, $\vv$
  must be sign-orthogonal on all cyclic {\flow}s $\modevectorcyc$
  (see section \ref{sec:metabolicmodels}).  As a test, we enumerate
  all elementary cyclic {\flow}s $\modevectorcyc$ (the columns of
  $\Cmat$, not limited to the support of $\vv$) that are conformal
  with $\vv$ (i.e.~that have positive or vanishing, but not negative
  fluxes on the support of $\vv$). Any such {\flow} indicates a
  constraint violation. To correct $\vv$, we compute the mean ratio
  $\xi = \langle \frac{v_l}{k_l} \rangle_{l \in
    \mbox{supp}(\vv,\modevectorcyc)}$ and replace $\vv$ by
  $\vv' = \vv - \xi\,\modevectorcyc$. The corrected {\flow} $\vv'$
  is sign-orthogonal\footnote{The proof is simple. If all ratios
    $v_l/k_l$ on the overlap of $\vv$ and $\modevectorcyc$ are
    identical, the corresponding elements are eliminated in $\vv$ and
    there remain no non-zero elements common to $\vv'$ and
    $\modevectorcyc$.  Otherwise, some of the $\vv'$ values on
    the remaining overlap are positive and others are negative. In
    both cases, $\vv'$ and $\modevectorcyc$ are
    sign-orthogonal.} on $\modevectorcyc$.
\item \textbf{Respecting the weak thermodynamic condition} The weak
  thermodynamic condition resembles the strong thermodynamic flux condition,
  but it only holds for active reactions. It states that for any
  non-zero flux, there must be a thermodynamic force in the same
  direction. To comply with this condition, a {\flow} $\vv$ must be
  sign-orthogonal on all cyclic test modes $\modevectorcyc$
  (i.e.~on all columns of $\Cmat$ whose supports are within the
  support of $\vv$).  To test this, we enumerate all elementary cyclic
  test modes $\modevectorcyc$.  If we find one that is
  conformal with $\vv$, this shows that the constraint is violated. To
  repair the constraint violation, we compute
  $\xi = \mbox{min}_{l \in \mbox{supp}(\vv,\modevectorcyc)}
  v_l/k_l$ and define the corrected {\flow}
  $\vv' = \vv - \xi\,\modevectorcyc$, which is sign-orthogonal
  on $\modevectorcyc$. The proof is simple: our correction
  makes (at least) one of the fluxes in the cycle (defined by
  $\modevectorcyc$) vanish, but it does not revert any
  fluxes. Thus, $\vv'$ and $\modevectorcyc$ are
  sign-orthogonal.
\item \textbf{Respecting the economic condition} Non-beneficial
  submodes can be found and removed in a similar manner.  We use
  the same test as for the weak thermodynamic constraints, but considering
  {\futile} modes $\modevectorfut$ instead of cyclic modes
  $\modevectorcyc$ as test modes.  The number of elementary
  {\nonbeneficial} modes can be large, which makes the calculation more
  expensive.
\end{enumerate}

\textbf{Remarks:} (i) In all three cases, we only need to check
\emph{elementary modes}. If a constraint is violated by a
non-elementary mode, it will also be violated by some elementary
mode. In contrast, if there are no constraint violations by any
elementary modes, there are also no constraint violations by any
non-elementary modes.  (ii) In all three cases, the correction
procedure can be run iteratively until no constraint violations
remain.  In the cases 2 and 3 (weak thermodynamic condition and economic
condition), this procedure removes all constraint violations (because
in every step, fluxes are switched off, while no fluxes change their
directions). In the first case (strong thermodynamic constraint), a
correction step may change some flux directions, and there is no proof
that the iterative procedure converges to a feasible flux profile.

\begin{figure*}[t!]
 \begin{center}
 \includegraphics[width=16cm]{\psfilesfluxes/corrections.eps}
 \caption{Infeasible patterns in metabolic {\flow}s can be detected and
   removed by inspecting elementary flux modes. We consider three
   types of constraint. (a) Strong thermodynamic constraints. (b) Weak
   thermodynamic constraints. (c) Economic constraints. }
 \label{fig:corrections}
 \end{center}
\end{figure*}

\coout{What about
  other conditions, for instance, more rows in Naug? Mention this in
  paper: everal objectives: adding more neutrality requirements =
  fewer elementary modes = helps to check for fluxes that optimise
  NONE of the alternative objectives?}

\subsection{Algebraic constraints on  {\fluxburden}s}
\label{sec:SIAlgConstraintFluxBurden}

\myparagraph{\ \\The {\fluxburden} vector $\hvv$ in an optimal state is
  orthogonal on all {\futile} flux modes}
We consider a model with a flux objective (i.e.~no cost effect of
metabolite concentrations). If $\vv$ is an economical {\flow} and $\vv_{\rm fut}$
is a {\futile} flux mode, the {\summationcondition} implies the equality 
\begin{eqnarray}
 \vv_{\rm fut}  \odots (\hudot \oslashs \vv) = 0.
\end{eqnarray}
This means that the flux {{\price} vector $\hvv = \hudot \oslashs \vv$ in
  an optimal state is orthogonal on all futile flux modes
  $\vv_{\rm fut}$. This holds, in particular, for all {\flow}s
  $\vv_{\rm fut} = \kv^{(1)}-\kv^{(2)}$, where $\kv^{(1)}$ and $\kv^{(2)}$
  are {\flow}s with identical flux benefit.

\paragraph{The {\fluxburden} vector $\hvv$ lies in the image space of $\Nobj\trans$}
Let $\Kobj$ be a maximal right-kernel matrix of
$\Nobj = {\bvtot\trans \choose \Nint }$, satisfying
$\Nobj\, \Kobj = 0$. Then any {\futile} flux vector $\vv_{\rm fut}$
can be written as a linear combination of the columns of $\Kobj$, and
the {\summationcondition} (for models with a flux objective) can be
written
\begin{eqnarray}
  \label{eq:loop5}
  \Kobj\trans (\hudot \oslashs \vv) = 0.
\end{eqnarray}
This means that  the {\fluxburden} vector $\hvv = \hudot \oslashs \vv$ must be a
linear combination of the columns of $\Nobj\trans$.


\subsection{How to compute economic potentials based on heuristic
  assumptions}
\label{sec:princdistribinvestment}

In the \fluxbenefitbalance \ref{eq:reactionbalanceeq}, a given
metabolic {\flow} $\vv$ constrains the economic potentials $\winti$, but it 
does not determine them precisely. This means that there is some freedom of
choice.  How can we choose plausible economic potentials,
i.e.~potentials that we expect to find in  realistic kinetic
models?  We assume that $\vv$ is economical, i.e.~that a solution for
$\wint$ exists.  To obtain a realistic solution, we can make heuristic
assumptions about the enzyme costs $\zcostgenerics_{l}$. We consider two
possibilities. We either assume that all enzymes have similar
costs (``postulate of uniform {{\enzymeinvestment}}s''), or assume some
predefined set of cost values and try to approximate it as closely as
possible with our economic potentials.  In networks with conserved
moieties, there will be some gauge freedom in choosing $\wint$
(right-kernel vectors of ${\Nint}\trans$ can be freely added); to
obtain a unique solution, an additional regularisation condition can 
be applied (e.g.~minimising the norm $||\wint||^2$).

\begin{itemize}[leftmargin=5mm]
\item \textbf{Economic potentials that correspond to uniform
    {{\enzymeinvestment}}s.}  Given an {\complete} economical metabolic {\flow}
  $\vv$ and a {\fluxgain} vector $\bvtot$, our aim is to find
  internal economic potentials $\wint$ and {{\enzymeinvestment}}s $\hudot$
  that satisfy the {\fluxbenefitbalance} and that agree with our
  heuristic assumptions.  Summing over all {\fluxbenefitbalance}s (and
  assuming that all reactions are enzyme-catalysed), we obtain the
  equality
 \begin{eqnarray}
 \label{eq:balancedinvestments1}
 \sum_{l} \zcostgenerics_{l} = \sum_{l} \partial \hul\, \ul = \sum_{l} [\Deltar \wintl + \bvtotl]\,v_{l} = \bvtot\cdot \,\vv.
 \end{eqnarray}
 To satisfy this equation by a choice of internal economic potentials
 $\wint$, we apply a assumption: all enzymes should have similar
 {\costshade}s. For deriving the formula, we first consider a
 simplified case.  If the {{\enzymeinvestment}}s could be freely varied, we
 could realise our assumption by minimising $\sum_{l} (\zcostgenerics_{l})^{2}$,
 the sum of squared {{\enzymeinvestment}}s, under the constraint
 $\sum_{l} \zcostgenerics_{l} = \bvtot\cdot \,\vv$. With a Lagrange multiplier
 $\alpha$, we can formulate this as
 \begin{eqnarray}
 \label{eq:balancedinvestments00}
 \mbox{Minimise}\; && \sum (\zcostgenerics_{l})^{2} - \alpha (\sum_{l} \zcostgenerics_{l} - \bvtot\cdot \,\vv).
 \end{eqnarray}
 The solution $\zcostgenerics_{l}= -\alpha/2 = \const$ shows that all
 {{\enzymeinvestment}}s are equal just as required. However, we cannot
 assume that the enzyme costs can be freely varied, because they
 depend on the economic potentials as
 $y_l = v_{l}\, [({\Nint}\trans\, \wint)_{l} + \bvtotl]$. Instead we
 use the internal economic potentials as free variables and obtain
 the variational principle
 \begin{eqnarray}
 \label{eq:balancedinvestments3}
 \mbox{Minimise}\; &&
 \sum (\zcostgenerics_{l})^{2} 
 = \sum_{l} \left(v_{l}\, [({\Nint}\trans\, \wint)_{l} + \bvtotl]\right)^{2}\qquad \mbox{w.r.t.}\quad \wint,
 \end{eqnarray}
where the {{\enzymeinvestment}}s must either be positive or
larger than some positive minimal value $\zcostgenerics_{l}^{\rm min}$:
 \begin{eqnarray}
 \label{eq:balancedinvestments4}
 \zcostgenerics_{l}^{\rm min} \le \zcostgenerics_{l} = v_{l} [\Deltar \wintl + \bvtotl].
 \end{eqnarray}
Altogether, we  obtain the quadratic optimality problem for $\wint$ 
 \begin{eqnarray}
 \label{eq:balancedinvestments4Opt}
 \mbox{Minimise}\; && {\wint}\trans\, \Nint\, \diag(\vv)^{2} {\Nint}\trans\, \wint
 + 2\, {\wint}\trans\, \Nint\, \diag(\vv)^{2}\,\bvtot \quad \mbox{w.r.t}\; \wint \nonumber \\
\mbox{subject to}
 &&\hudotmin \cdot {{\bf 1}} - \diag(\vv)\, \bvtot \le \diag(\vv)\,{\Nint}\trans \wint,
 \end{eqnarray}
 where ${{\bf 1}} = (1, 1, ..)\trans$.  \coout{ \footnote{ \co{Without
       the constraints, the solution would read
   \begin{eqnarray}
 \label{eq:balancedinvestments4a}
 \wint = - \left(\Nint\, \diag(\vv)^{2}\, \Nint\right)\inv \Nint\, \diag(\vv)^{2}\, \bvtot.
 \end{eqnarray}
 if the matrix $\Nint\, \diag(\vv)^{2} {\Nint}\trans$ is
 invertible. If this is not the case, then to pick a specific
 solution, the matrix inverse can be replaced by the
 pseudo-inverse.}}.}  In models with moiety conservation, the matrix
$\Nint\, \diag(\vv)^{2} {\Nint}\trans$ is not invertible, so the
solution will not be unique.  For a unique solution, we can add a
regularisation term, e.g.~$\beta ||{\wint}||^{2}$ with a small
prefactor $\beta$. The calculation works only for {\complete} flux
profiles; inactive reactions must be omitted from the model.

\item \textbf{Economic potentials that correspond ro given enzyme
    costs or {\fluxburden}s.} As another heuristics, we may fit the
  economic potentials to given {{\enzymeinvestment}}s $\zcostgenerics_{l}^{\rm
    data}$. Given the predefined fluxes and {\fluxgain}s, we first
  scale the presumable {\enzymeinvestment}s $\zcostgenerics_{l}^{\rm data}$ to satisfy
  the sum rule $\sum_{l} \zcostgenerics_{l}^{\rm data} = \bvtot\cdot \,\vv$
  (Eq.~(\ref{eq:balancedinvestments1})). Then, to compute the economic
  potentials we postulate that the ratios $\zcostgenerics_{l}/\zcostgenerics_{l}^{\rm data}$
  must be similar for all enzymes. We implement this by the principle
  of known {\enzymeinvestment}s
 \begin{eqnarray}
 \label{eq:balancedinvestments5}
\mbox{Minimise}\;
 \sum \frac{(\zcostgenerics_{l})^{2}}{\zcostgenerics_{l}^{\rm data}} \qquad \mbox{subject to}\quad\sum \zcostgenerics_{l} = \sum_{l} \zcostgenerics_{l}^{\rm data}.
 \end{eqnarray}
 We obtain a slightly different quadratic
 optimality problem for $\wint$, with the same constraints:
\begin{eqnarray}
 \label{eq:balancedinvestments6}
\mbox{Minimise}\;
&& {\wint}\trans\, \Nint\, \diag(\vv)^{2}\, \diag({\hudot}^{\rm data})\inv {\Nint}\trans\, \wint
 + 2\, {\wint}\trans\, \Nint\, \diag(\vv)^{2}\,\diag({\hudot}^{\rm data})\inv\,\bvtot \nonumber \\
\mbox{subject to}
 &&\hudotmin \cdot {{\bf 1}} - \diag(\vv)\, \bvtot \le \diag(\vv)\,{\Nint}\trans \wint.
\end{eqnarray}
Again, regularisation may be used to obtain unique solutions in models
with moiety conservation.  By inserting our result $\wint$ into the
{\fluxbenefitbalance}, we obtain the {{\enzymeinvestment}}s $\hudot$, which
approximate the predefined {{\enzymeinvestment}}s ${\hudot}^{\rm data}$.  This
principle can be applied in various ways: (i) we can start from
presumable {\enzymeinvestment}s obtained from protein sizes and proteomics
data (see section \ref{sec:potentaislfromenzymepar}); (ii) we can
require uniform {\enzymeinvestment}s across all enzymes (and reobtain our
previous heuristics); (iii) we can assume given or uniform flux
{\price}s $\hvl^{\rm data}$ (estimated from protein properties alone;
see \ref{sec:potentaislfromenzymepar}) and set
$\zcostgenerics_{l}^{\rm data} = \hvl^{\rm data}\,v_l$; or (iv) the algorithm can
be applied to randomly sampled {{\enzymeinvestment}}s ${\hudot}^{\rm data}$ to
obtain an ensemble of enzyme-balanced models.

\end{itemize}

\subsection{How to estimate enzyme costs from enzyme molecule properties}
\label{sec:potentaislfromenzymepar}

\myparagraph{\ \\Estimation of {{\enzymeinvestment}}s} How can we estimate
the {{\enzymeinvestment}}s $\zcostgenerics_{l}=\hul\,\ul$ from measured metabolic flux and
proteome data?  We assume that the costs are proportional to
measured enzyme levels $e^{\rm data}_{l}$. For the {{\enzymeprice}}s, we
assume a proportionality
\begin{eqnarray}
\label{eq:enzymeparametersandforce1}
\hul \sim L_{l}\,(\lambda + \enzdegrate_{l})
\end{eqnarray}
with enzyme sizes $L$ (number of amino acids), cell growth rate
$\lambda$, and enzyme degradation rates $\enzdegrate_l$
\cite{lieb:14a}.  For the absolute scaling, we can rescale the
{\enzymeinvestment}s by a prefactor
$\frac{\bvtot\cdot \vv}{\sum_{l}\, \zcostgenerics_{l}^{\rm data}}$. The rescaled
{\enzymeinvestment}s will sum to the total flux benefit $\bvtot\cdot \vv$.

\myparagraph{Estimation of {\fluxvalue}s from enzyme parameters} In
kinetic models the economic potentials $\wtoti$ and {{\enzymeprice}}s
$\hul$ are related to enzyme kinetics and, in particular, to the
catalytic constants $\kcat$.  How can we use known catalytic constants
to estimate the economic potentials?  In enzyme-optimal states, the
equation $\Deltar \wtot + \bvdir = \hvv$ must be satisfied. The flux
{\burden}s $\hvs = \hus\,u/v$ are state-dependent and thus variable,
but in any case they need to satisfy some constraints.  A reaction
rate is given by $\rate(\cv)=u\,\ratelaw(\cv)$ with an enzyme
efficiency $\ratelaw$ in the range
$-k^{\rm cat-} \le \ratelaw \le k^{\rm cat}$. If we assume a positive
flux, the flux can be approximated by
\begin{eqnarray}
\label{eq:enzymeparametersandforce2}
\hvs = \frac{\hus}{\ratelaw} = \alpha_{\rm scale} \frac{L\,(\lambda + \enzdegrate)}{\ratelaw}
\ge \alpha_{\rm scale} \frac{L\,(\lambda + \enzdegrate)}{k^{\rm cat}\,(1-\e^{\Deltar G/RT})}.
\ge \alpha_{\rm scale} \frac{L\,(\lambda + \enzdegrate)}{k^{\rm cat}},
\end{eqnarray}
where $\lambda + \enzdegrate$ is the proteins's effective degradation
constant, $L$ is its amino acid chain length, and $\alpha_{\rm scale}$ is a
scaling factor. To determine $\alpha_{\rm scale}$, we set the sum
$\sum_{l} \hvl\,v_{l}$ equal to the total {{\enzymeinvestment}}, $y_{\rm tot} =
\sum_l \hvl \, v_l = \alpha_{\rm scale} \sum_l \frac{L\,(\lambda +
  \kappa)\,v_l}{k^{\rm cat}}$, and obtain $\alpha_{\rm scale} = \frac{y_{\rm
    tot}}{\sum_l \frac{L\,(\lambda + \enzdegrate)\,v_l}{k^{\rm cat}}}$.
When an enzyme operates at its maximal  speed, its specific rate is given by
$\ratelaw_{l} = k^{\rm cat}_{+}$ (or, in the case of negative fluxes,
$\ratelaw_{l} = -k^{\rm cat}_{-}$).  In VBA, the expressions in
Eq.~(\ref{eq:enzymeparametersandforce2}) can be used to estimate or
delimit the   {\fluxburden}s $\hvl=\zcostgenerics_{l}/v_{l}$ or
the {\fluxvalue}s $\Deltar \wtotl + \bvdirl$.

 \myparagraph{Correction of estimated {\fluxburden} based on
   {\summationconnectivitycondition}} To estimate $\hvv$ by equation
 (\ref{eq:enzymeparametersandforce2}), we need to know the flux directions, but
 not the quantitative fluxes. If the fluxes $v_{l}$,
 enzyme levels $\ul$, and enzyme {\price}s $\hul$ are known, we can determine
 the {\fluxburden}s $\hvl = \hul \frac{\ul}{v_{l}}$. However, the data values (fluxes or enzyme levels) are typically imprecise,. In this case,
 additional constraints on $\hvv$ can be used to improve
 our estimates. To satisfy  the flux benefit balance, {\fluxburden}s
 $\hvl$ and {\fluxgain}s $\bvtotl$ must satisfy the condition
\begin{eqnarray}
\hvv - \bvtot = {\Nint}\trans {\wint}\trans \in \mbox{Span}({\Nint}\trans).
\end{eqnarray}
Measured or estimated {\fluxburden}s are likely to  violate this
equation. To correct them, we compute  the
left-hand side and project it onto the hyperplane spanned by the columns of
${\Nint}\trans$.  From the {\fluxgain} condition
Eq.~(\ref{eq:fitnessbalance2}), we obtain similar constraints: the
vector $\hvv$ must be orthogonal on all {\futile} flux test modes
$\kv_{\rm fut}$. 
If we define $\Nobj = {{\bvtot}\trans \choose \Nint}$, and
its kernel matrix $\Kobj$ satisfying
${{\bvtot}\trans \choose \Nint} \,\Kobj=0$, then ${\hvv}$ must satisfy
${\hvv}\trans\,\Kobj=0$ and must thus be a linear combination of the
columns of $\Nobj\trans$.  In models with a pure concentration
objective (i.e.~$\bvtot=0$), the vector $\hvv$ must be orthogonal on
\emph{all} stationary {\flow}s, i.e.~it must be a linear combination of
the columns of ${\Nint}\trans$.  Finally, the {\fluxburden}s must
satisfy the {\connectivitycondition} \cite{lieb:14a}
\begin{eqnarray}
\label{eq:constraintforfluxprices}
(\Eunint\,\Lmat)\trans\,\hvv = -\Lmat\trans\,\bc
\end{eqnarray}
with the unscaled elasticity matrix $\Eunint$ and the link matrix
$\Lmat$.  In contrast, in models with a pure flux objective
(i.e.~$\bc = 0$), the {\fluxburden} vector $\hvv$ must be orthogonal
on all columns of $\Eunint\, \Lmat$. In linear pathways, this yields a
direct  relationship between elasticities and flux
{\burden}s in the same reactions.
From the estimated {\fluxburden}s $\hvl^{\rm est}$, we can
determine corrected {\fluxburden}s $\hvl$ by a least-squares
regression (requiring $\hvl \stackrel{!}{\approx} \hvl^{\rm est}$) under the
constraints given by Eq.~(\ref{eq:constraintforfluxprices})).

\myparagraph{Conversion of {\fluxvalue}s into economic potentials}
If the {\fluxvalue}s $\gvtotl$ in a model are known, they will
constrain the economic potentials $\winti$. To determine a single
solution, we can pick one of them by minimising the Euclidean norm
$||\winti||$ under the constraint
$\gvtotl = \Deltar \wtotl + \bvdirl$.  If also the fluxes are given,
there is a second possibility: we may translate $\gvtotl$ into the
{{\enzymeinvestment}s} ${\zcostgenerics}_{l} = \gvtotl \,v_{l}$ and proceed as
described in section \ref{sec:princdistribinvestment}.  If lower
bounds $\zcostgenerics^{\rm min}$ are known, we first need to check that the
constraint $\zcostgenerics_{l}> \zcostgenerics_{l}^{\rm min}$ is satisfied.

  \section{Fluxes and potentials in the PFK/FBPase cycle}

  \co{ist der abschnitt gut? dann ref in main text!} \todo{The
    possible fluxes in the PFK/FBP system are closely related to the
    chemical and economic potentials. The fact that PFK is only used
    for glycolysis and FBPase is only used for gluconeogenesis can be
    understood by combining thermodynamic and economic constraints.
    Since both reactions can theoretically run in forward or reverse
    direction or be shut off, we obtain nine possible sign
    combinations, two of which correspond to the typical fluxes in
    glycolysis (PFK foward/FBPase off) and glyconeogenesis (PFK
    off/FBPase forward). In fact, under relatively general
    assumptions, all other sign combinations can be ruled out by the
    thermodynamic and economic constraints. If we assume that the ATP
    has a higher chemical potential and a higher economic potential
    than ADP, three out of nine possible sign combinations can be
    excluded. And under physiological conditions, either PFK or FBPase
    is active (each in forward direction), or both are shut off.

To study this in more detail, we list all possible flux patterns and check
them for thermodynamic and economic feasibility.  We consider the
potentials of four metabolites ADP (plus inorganic phosphate; denoted
by A), ATP (plus water; denoted by B), as well as F6P (X) and FBP
(Y). We assume that under all physiological conditions, ADP (plus
phosphate) has a lower chemical potential $\mu_{A}<\mu_{B}$ than ATP
(plus water), and also a lower economic potential $w_{A}<w_{B}$. For
the chemical potentials of F6P and FBP, we also consider three
possible cases:
\begin{center}
 \begin{tabular}{llll}
   Case & Condition & (PFK/FBP) \\ 
   ($\alpha$) & $\mu_{X}<\mu_{Y}$                                      & infeasible & feasible \\ 
   ($\beta$)  & $\mu_{X}>\mu_{Y}$ but  $\mu_{X}+\mu_{A}<\mu_{Y}+\mu_{B}$  & infeasible & infeasible\\ 
   ($\gamma$) & $\mu_{X}+\mu_{A}<\mu_{Y}+\mu_{B}$                        & feasible & infeasible \\
 \end{tabular}
\end{center}
Likewise, for the economic potentials of F6P and FBP, we consider
three possible cases
\begin{center}
\begin{tabular}{llll}
  Case & Condition & PFK & FBPase \\ 
  (A) & $w_{X}<w_{Y}$                               & beneficial & \wasteful \\  
  (B) & $w_{X}>w_{Y}$, but $w_{X}+w_{A}<w_{Y}+w_{B}$   & beneficial & beneficial \\
  (C) & $w_{X}+w_{A}>w_{Y}+w_{B}$                     & \wasteful & beneficial
\end{tabular}
\end{center}
Altogether, we obtain nine possible scenrios.  Now we consider all
possible flux patterns and ask which of these scenarios they can be
realised. Note that vanishing fluxes are always allowed.

\begin{center}
\begin{tabular}{l|lll}
  & $v_{PFK} <0$        & $v_{PFK} =0$              & $v_{PFK} >0$            \\ 
\hline
  $v_{FBP}>0$  & case $\alpha$C       & cases $\alpha$B, $\alpha$C        & thermodynamically infeasible \\
  $v_{FBP}=0$  & cases $\alpha$C, $\beta$C  & always possible         & cases $\gamma$A, $\gamma$B     \\
  $v_{FBP}<0$  & economically infeasible & cases $\beta$A, $\gamma$A   &  case $\gamma$A       
\end{tabular}
\end{center}

Thus, the two cycle fluxes (PFK and FBPase both active in forward
direction, or both in reverse direction) are infeasible. The fluxes in
which both enzymes are active, either in glycolytic or gluconeogenic
direction are theoreticall feasible, but only under physiologically
unusual circumstances.

\begin{figure*}[h!]
  \begin{center}
\parbox{11cm}{\includegraphics[width=10.5cm]{\psfilesfluxes/pfk_example.eps}}
\parbox{5cm}{ 
%  \[ \Delta \mu_{\rm F} = \mu_{\rm FBP} - \mu_{\rm F6P}\]
%  \[ \Delta \wint_{\rm F} = \wint_{\rm FBP} - \wint_{\rm F6P}\]
%  \[ \Delta \mu_{\rm A} = \mu_{\rm ATP} - \mu_{\rm ADP}\]
%  \[ \Delta \wint_{\rm A} = \wint_{\rm ATP} - \wint_{\rm ADP} \]
% 
\coout{inaktive reaktionen in graphik gestrichelt zeigen}
 Energy and economic potential differences
 \begin{eqnarray*}
 \mu_{\rm PFK}    &=& \Delta \mu_{\rm F} - \Delta \mu_{\rm A} \\
   \wsymbol_{\rm PFK}    &=& \Delta   \wsymbol_{\rm F} - \Delta   \wsymbol_{\rm A} \\
 \mu_{\rm FBPase} &=& - \Delta \mu_{\rm F} \\
   \wsymbol_{\rm FBPase} &=& - \Delta   \wsymbol_{\rm }
 \end{eqnarray*}
}
\caption{\co{compare picture to table above. which one is better?}
  Thermodynamic and economic constraints in the PFK/FBPase loop.  (a)
  The enzymes phosphofructokinase (PFK) and fructose bisphosphatase
  (FBPase) can catalyse an ATP-consuming substrate cycle, but the flux
  cycle is usually suppressed in living cells.  (b) Feasible flux
  patterns.  According to VBA, the flux directions must agree
  with the differences between chemical potentials $\mu_{i}$ and
  economic potentials $\wsymbol_{i}$ along the reactions. The
  conversion from ATP to ADP requires a decrease
  $\Delta \mu_{\rm A} = \mu_{\rm ATP} - \mu_{\rm ADP}$ in chemical
  potential and amn increase
  $\Delta \wsymbol_{\rm A} = \wsymbol_{\rm ATP} - \wsymbol_{\rm ADP}$
  in economic potential.  In contrast, the differences
  $\Delta \mu_{\rm F} = \mu_{\rm FBP} - \mu_{\rm F6P}$ and
  $\Delta \wsymbol_{\rm F} = \wsymbol_{\rm FBP} - \wsymbol_{\rm F6P}$
  may depend on the situation. The table shows the feasible fluxes for
  different possible combinations. Feasible forward and reverse fluxes
  and mandatory zero fluxes are indicated by +, -, and 0 (where fluxes
  with a predefined sign are also allowed to vanish). If reactions
  have no direct {\fluxvalue}, and with physiologically plausible
  values for $\Delta \mu_{l}$ (centre column), the two enzymes cannot
  be active at the same time.}
    \label{fig:pfk_example}
  \end{center}
\end{figure*}

How would other flux prediction methods describe the PFK/FBPase
system?  FBA without sign constraints would yield another, must less
realistic result. it would predict the cycle to run in reverse
direction, converting inorganic phosphate into ATP, which is
thermodynamically impossible under physiological conditions.
Thermodynamic FBA, with realistic chemical potentials of ATP, ADP, and
inorganic phosphate, woudl avoid this cycle, but it would allow the
ATP-saving reverse use of FBPase for glycolysis; only if all chemical
potentials for both situations (glycolysis and gluconeogenesis) are
given, all wrong solutions are excluded, but this is trivial since the
flux directions would be predefined.}


